Charm Production and QCD Analysis at HERA and LHC

This review is devoted to the study of charm production in ep and pp collisions. The total set of measurements obtained by the two collaborations H1 and ZEUS from HERA and their combination is outlined, as well as complementary data obtained by the LHCb collaboration at the LHC. After fitting the parton distribution functions the charm production cross sections are predicted within perturbative QCD at next-to-leading order using the fixed-flavour-number scheme. Agreement with the data is found. The combined HERA charm data are sensitive to the $c$-quark mass and enabled its accurate determination. The predictions crucially depend upon the knowledge of the gluon distribution function. It is shown that the shape of the gluon distribution based on the HERA data is considerably improved by adding the measurements from LHCb and applicable down to values x of about 10^{-6}, where x is the proton momentum fraction carried by a parton.

==> content/combination/dstar/cs/combinedfull1.tex <==
%\begin{sidewaystable}[tbp]
\begin{table*}[tbp]
\footnotesize
%\begin{center}
\tabcolsep0.15mm
\renewcommand*{\arraystretch}{1.0}
\begin{tabu} to \textwidth{|>{$}c<{$}|>{$}l<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|} \hline
p_T(\Dstar)&\frac{{\rm d}\sigma}{{\rm d}p_T(\Dstar)}&\delta_{unc}&\delta_1&\delta_2&\delta_3&\delta_4&\delta_5&\delta_6&\delta_7&\delta_8&\delta_9&\delta_{10}&\delta_{11}&\delta_{12}&\delta_{13}&\delta_{14}&\delta_{15}&\delta_{16}&\delta_{17}&\delta_{18}&\delta_{19}&\delta_{20}&\delta_{21}&\delta_{22}&\delta_{br} \\
%[$\SI{}{GeV}$]&[$\SI{}{nb/GeV}$]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%] \\ \hline
$[\SI{}{GeV}]$&$[\SI{}{nb/GeV}]$&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%] \\ \hline
 1.50: 1.88&   2.358&   6.4&  -0.4&   0.8&   0.8&  -1.0&   0.4&   0.0&  -1.8&   0.3&   0.1&  -1.0&   0.6&   1.0&  -0.1&   0.7&   0.6&  -0.4&  -1.4&   0.2&  -0.5&  -0.8&  -2.7&   0.4&   1.5 \\ 
 1.88: 2.28&   2.227&   4.8&  -0.5&   0.5&   0.7&  -0.9&   0.3&   0.0&  -1.9&   0.3&   0.2&  -1.0&   0.6&   0.8&  -0.2&   0.6&   0.5&  -0.4&  -1.0&   0.5&  -0.3&  -0.4&  -2.1&   0.3&   1.5 \\ 
 2.28: 2.68&   1.984&   3.7&  -0.4&   0.6&   0.5&  -0.9&   0.3&   0.0&  -1.9&   0.3&   0.2&  -1.0&   0.7&   1.0&  -0.1&   0.7&   0.4&  -0.3&  -0.9&   0.5&  -0.5&  -0.0&  -1.7&   0.6&   1.5 \\ 
 2.68: 3.08&   1.559&   3.5&  -0.4&   0.6&   0.5&  -0.8&   0.3&   0.0&  -1.9&   0.3&   0.2&  -1.0&   0.6&   1.0&  -0.2&   0.7&   0.4&  -0.8&  -0.5&   0.2&  -0.2&   0.2&  -0.9&   0.4&   1.5 \\ 
 3.08: 3.50&   1.209&   3.6&  -0.4&   0.6&   0.5&  -0.8&   0.3&   0.0&  -1.8&   0.2&   0.1&  -0.9&   0.7&   1.1&  -0.3&   0.5&   0.3&  -0.4&  -0.4&   0.3&  -0.1&   0.1&  -0.7&   0.3&   1.5 \\ 
 3.50: 4.00&   0.9328&   3.2&  -0.4&   0.7&   0.3&  -0.8&   0.3&   0.0&  -1.7&   0.2&   0.0&  -0.9&   0.7&   1.0&  -0.2&   0.6&   0.3&  -0.4&  -0.3&   0.0&  -0.2&   0.1&  -0.7&   0.4&   1.5 \\ 
 4.00: 4.75&   0.6161&   3.0&  -0.4&   0.6&   0.3&  -0.7&   0.3&   0.0&  -1.7&   0.1&  -0.0&  -0.9&   0.8&   1.1&  -0.1&   0.5&   0.5&  -0.4&  -0.2&   0.4&   0.0&   0.6&   0.6&   0.0&   1.5 \\ 
 4.75: 6.00&   0.3204&   3.0&  -0.4&   0.6&   0.3&  -0.7&   0.3&   0.0&  -1.6&   0.1&  -0.1&  -0.9&   0.8&   1.0&  -0.2&   0.6&   0.3&  -0.3&  -0.0&   0.1&  -0.2&   0.5&  -0.4&   0.3&   1.5 \\ 
 6.00: 8.00&   0.1152&   3.8&  -0.3&   0.7&   0.2&  -0.6&   0.2&   0.0&  -1.6&   0.1&  -0.0&  -0.9&   0.6&   1.1&  -0.2&   0.5&   0.2&  -0.0&  -0.2&   0.4&   0.5&   1.3&   1.0&  -0.3&   1.5 \\ 
 8.00:11.00&   0.03334&   5.3&  -0.3&   0.7&   0.3&  -0.7&   0.3&   0.0&  -1.5&   0.1&  -0.1&  -0.9&   0.7&   1.0&  -0.1&   0.1&   0.4&   0.5&  -0.3&  -0.1&  -0.6&   1.4&  -1.1&   0.2&   1.5 \\ 
11.00:20.00&   0.003819&  10.3&  -0.3&   0.6&   0.5&  -0.8&   0.4&   0.0&  -1.4&   0.1&  -0.0&  -0.8&   0.5&   1.1&   0.1&   0.1&   0.1&   0.7&   0.2&  -1.6&  -0.6&   0.8&  -5.1&   1.4&   1.5 \\ \hline
\hline
\eta(\Dstar)&\frac{{\rm d}\sigma}{{\rm d}\eta(\Dstar)}&\delta_{unc}&\delta_1&\delta_2&\delta_3&\delta_4&\delta_5&\delta_6&\delta_7&\delta_8&\delta_9&\delta_{10}&\delta_{11}&\delta_{12}&\delta_{13}&\delta_{14}&\delta_{15}&\delta_{16}&\delta_{17}&\delta_{18}&\delta_{19}&\delta_{20}&\delta_{21}&\delta_{22}&\delta_{br} \\ 
&[$\SI{}{nb}$]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%] \\ \hline
-1.50:-1.25&   1.360&   5.8&   1.1&   1.2&  -0.5&  -1.1&  -0.9&  -0.0&  -0.6&  -0.5&   0.3&  -0.2&  -0.3&  -0.0&  -0.1&   0.1&   0.6&   0.6&  -0.9&  -0.9&   1.2&  -2.5&  -0.6&  -0.1&   1.5 \\ 
-1.25:-1.00&   1.515&   4.6&   1.0&   1.3&  -0.4&  -0.9&  -0.7&  -0.0&  -0.4&  -0.5&   0.4&  -0.2&  -0.3&  -0.2&   0.4&   0.5&   0.7&   0.8&  -0.7&  -1.1&   0.9&  -1.9&  -0.8&   0.0&   1.5 \\ 
-1.00:-0.75&   1.587&   4.6&   1.0&   1.3&  -0.4&  -0.9&  -0.7&  -0.0&  -0.4&  -0.5&   0.5&  -0.3&  -0.3&  -0.2&   0.4&   0.7&   0.7&   0.6&  -1.0&  -1.1&   0.8&  -1.6&  -1.3&   0.0&   1.5 \\ 
-0.75:-0.50&   1.789&   3.8&   1.1&   1.3&  -0.3&  -1.0&  -0.6&  -0.0&  -0.4&  -0.5&   0.4&  -0.2&  -0.3&  -0.1&   0.2&   0.4&   0.5&   0.4&  -0.7&  -0.7&   0.6&  -1.7&  -0.6&   0.2&   1.5 \\ 
-0.50:-0.25&   1.833&   3.8&   1.1&   1.2&  -0.3&  -1.0&  -0.6&  -0.0&  -0.3&  -0.6&   0.3&  -0.1&  -0.2&  -0.1&   0.1&   0.3&   0.5&   0.2&  -0.6&  -0.7&   0.5&  -1.6&   0.3&  -0.0&   1.5 \\
-0.25: 0.00&   1.887&   3.8&   1.2&   1.3&  -0.2&  -1.0&  -0.5&  -0.0&  -0.3&  -0.5&   0.4&  -0.1&  -0.2&  -0.1&   0.0&   0.2&   0.6&   0.4&  -0.7&  -0.6&   0.9&  -1.4&  -1.5&   0.3&   1.5 \\ 
 0.00: 0.25&   1.857&   4.0&   1.2&   1.3&  -0.2&  -1.0&  -0.5&  -0.0&  -0.3&  -0.6&   0.4&  -0.1&  -0.1&  -0.1&   0.0&  -0.0&   0.1&   0.4&  -0.3&  -0.5&   0.5&  -1.6&   1.0&  -0.1&   1.5 \\ 
 0.25: 0.50&   1.879&   4.0&   1.1&   1.3&  -0.2&  -1.0&  -0.5&  -0.0&  -0.2&  -0.5&   0.5&  -0.1&  -0.1&  -0.1&   0.2&   0.1&   0.5&   0.7&  -0.6&  -0.5&   0.8&  -1.4&  -1.4&   0.3&   1.5 \\
 0.50: 0.75&   1.909&   4.1&   1.1&   1.3&  -0.2&  -1.0&  -0.5&  -0.0&  -0.3&  -0.5&   0.5&  -0.1&  -0.1&  -0.1&   0.2&   0.3&   0.5&   0.4&  -0.8&  -0.6&   0.5&  -1.6&  -0.9&   0.2&   1.5 \\ 
 0.75: 1.00&   1.920&   4.3&   1.1&   1.3&  -0.2&  -1.0&  -0.5&  -0.0&  -0.3&  -0.5&   0.4&  -0.1&  -0.1&  -0.1&   0.2&   0.3&   0.4&   0.8&  -1.3&  -0.6&   0.6&  -1.8&  -1.6&   0.2&   1.5 \\ 
 1.00: 1.25&   2.075&   4.7&   1.1&   1.3&  -0.2&  -0.9&  -0.5&  -0.0&  -0.3&  -0.6&   0.4&  -0.2&  -0.1&  -0.2&   0.2&   0.2&   0.7&   0.7&  -1.0&  -0.4&   0.3&  -2.3&   1.3&  -0.3&   1.5 \\ 
 1.25: 1.50&   1.813&   6.3&   1.0&   1.4&  -0.3&  -0.9&  -0.5&  -0.0&  -0.3&  -0.5&   0.4&  -0.2&  -0.2&  -0.2&   0.4&   0.6&   0.7&   0.7&  -1.4&  -1.3&   0.4&  -2.0&  -2.5&   0.2&   1.5 \\ \hline
\hline
z(\Dstar)&\frac{{\rm d}\sigma}{{\rm d}z(\Dstar)}&\delta_{unc}&\delta_1&\delta_2&\delta_3&\delta_4&\delta_5&\delta_6&\delta_7&\delta_8&\delta_9&\delta_{10}&\delta_{11}&\delta_{12}&\delta_{13}&\delta_{14}&\delta_{15}&\delta_{16}&\delta_{17}&\delta_{18}&\delta_{19}&\delta_{20}&\delta_{21}&\delta_{22}&\delta_{br} \\ 
&$[\SI{}{nb}]$&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%] \\ \hline
0.000:0.100&   3.277&   9.5&   1.7&   1.9&  -0.0&   1.1&   0.5&  -1.0&   1.0&   0.5&  -0.9&   0.4&   0.2&   0.7&   0.1&   0.1&  -0.1&  -1.1&   3.4&  -2.0&   1.1&  -1.3&   0.7&   0.6&   1.5 \\ 
0.100:0.200&   7.346&   4.8&   1.8&   1.2&  -0.2&   1.1&   0.2&  -1.0&   0.8&   0.4&  -0.7&   0.1&   0.3&   0.7&   0.4&   0.1&   0.3&  -1.4&   2.5&  -1.5&   2.9&  -2.9&   0.9&   0.8&   1.5 \\ 
0.200:0.325&   8.612&   3.5&   2.0&   1.0&  -0.1&   0.9&   0.2&  -0.6&   0.6&   0.5&  -0.2&   0.1&   0.3&   0.5&   0.6&   0.1&   0.3&  -1.2&   2.0&   0.3&   0.9&  -2.0&   0.6&   0.5&   1.5 \\ 
0.325:0.450&   8.918&   2.7&   2.1&   1.0&  -0.1&   0.9&   0.2&  -0.4&   0.4&   0.5&  -0.0&   0.0&   0.4&   0.4&   0.6&  -0.0&   0.3&  -0.7&   1.6&   1.2&  -0.7&  -0.3&   0.0&   0.3&   1.5 \\ 
0.450:0.575&   8.827&   1.8&   2.3&   1.2&   0.0&   0.8&   0.4&  -0.0&   0.3&   0.5&   0.3&   0.0&   0.4&   0.3&   0.4&  -0.1&   0.3&  -0.4&   0.7&   1.6&   0.9&  -0.1&  -0.1&   0.8&   1.5 \\ 
0.575:0.800&   4.785&   2.4&   2.2&   1.4&   0.1&   0.9&   0.6&  -0.0&   0.6&   0.5&   0.2&   0.1&   0.6&   0.4&   0.1&  -0.1&   0.2&   0.8&  -0.5&   2.5&   2.5&   0.4&  -0.5&   0.7&   1.5 \\ 
0.800:1.000&   0.6308&   8.1&   1.6&   0.8&  -0.3&   2.4&   1.0&  -1.5&   1.5&   0.2&  -1.3&  -0.2&   1.3&   1.0&  -0.3&  -0.1&   0.9&   3.8&  -2.8&   3.8&   4.4&   4.0&   3.1&  -0.4&   1.5 \\ \hline
\hline
Q^2&\frac{{\rm d}\sigma}{{\rm d}Q^2}&\delta_{unc}&\delta_1&\delta_2&\delta_3&\delta_4&\delta_5&\delta_6&\delta_7&\delta_8&\delta_9&\delta_{10}&\delta_{11}&\delta_{12}&\delta_{13}&\delta_{14}&\delta_{15}&\delta_{16}&\delta_{17}&\delta_{18}&\delta_{19}&\delta_{20}&\delta_{21}&\delta_{22}&\delta_{br} \\
$[\SI{}{GeV^2}]$&$[\SI{}{nb/GeV^2}]$&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%] \\ \hline
   5:   8&   0.4735&   4.0&   1.4&  -1.4&  -0.9&   0.9&  -0.9&   0.6&  -0.9&  -0.3&   1.1&  -0.2&   0.9&  -1.3&   0.7&   0.7&   0.8&   1.5&  -1.0&  -0.6&   0.7&  -2.1&  -1.2&   0.3&   1.5 \\ 
   8:  10&   0.2964&   4.3&   1.2&  -1.3&  -0.7&   0.7&  -1.0&   0.8&  -0.6&  -0.4&   1.0&   0.0&   0.8&  -1.0&   0.7&   0.4&   1.1&   1.1&  -0.2&  -0.1&  -0.1&   0.5&  -0.5&  -0.1&   1.5 \\ 
  10:  13&   0.2117&   3.8&   0.8&  -1.9&  -0.8&   0.8&  -0.6&   0.8&  -0.5&  -0.6&   1.0&  -0.1&   0.6&  -0.6&   0.4&  -0.1&   0.9&   1.0&  -0.9&   0.7&  -0.3&  -1.2&  -0.5&   0.4&   1.5 \\ 
  13:  19&   0.1236&   3.2&   0.8&  -1.8&  -0.8&   0.8&  -0.7&   0.8&  -0.4&  -0.7&   1.0&  -0.1&   0.6&  -0.6&   0.6&   0.0&   0.8&   0.8&  -0.0&   0.0&  -1.0&  -0.9&  -0.3&   0.5&   1.5 \\
  19:  28&   0.07263&   3.5&   0.8&  -1.8&  -0.7&   0.7&  -0.7&   0.8&  -0.3&  -0.7&   0.9&  -0.1&   0.6&  -0.6&   0.5&   0.2&   0.7&   0.7&  -0.0&   0.2&  -0.9&  -0.6&  -0.3&   0.4&   1.5 \\ 
  28:  40&   0.03970&   3.7&   0.7&  -1.9&  -0.8&   0.8&  -0.6&   0.8&  -0.3&  -0.8&   1.0&  -0.2&   0.5&  -0.5&   0.3&   0.0&   0.8&   0.6&  -0.6&   0.5&  -0.7&  -1.7&  -0.3&   0.6&   1.5 \\ 
  40:  60&   0.01635&   4.4&   0.7&  -2.0&  -0.8&   0.8&  -0.5&   0.7&  -0.3&  -0.7&   0.8&  -0.3&   0.6&  -0.4&   0.6&  -0.4&   0.5&   0.9&   0.5&  -0.0&  -1.5&  -2.6&  -0.6&   0.7&   1.5 \\ 
  60: 100&   0.007445&   5.2&   0.8&  -1.9&  -0.8&   0.9&  -0.5&   0.7&  -0.4&  -0.6&   0.9&  -0.3&   0.6&  -0.4&   0.7&  -0.3&   0.1&   0.2&   0.2&   0.9&  -1.6&  -0.4&   0.3&  -0.0&   1.5 \\ 
 100: 158&   0.002081&   7.2&   0.1&  -2.3&  -0.4&  -0.6&  -0.8&   0.3&  -0.2&  -0.8&   1.0&   0.0&   0.6&  -0.0&  -0.4&  -1.3&   0.7&   0.8&  -1.6&   1.8&  -2.5&  -0.8&  -1.3&  -0.5&   1.5 \\ 
 158: 251&   0.0008817&   7.6&   0.3&  -1.8&  -0.5&  -0.4&  -0.9&   0.2&  -0.4&  -0.8&   1.1&  -0.0&   0.7&  -0.3&  -0.0&  -1.0&   1.1&   0.0&  -0.2&   2.1&  -2.1&  -0.8&  -2.0&  -0.6&   1.5 \\ 
 251:1000&   0.0000749&  11.4&  -0.1&  -2.3&  -0.6&  -0.4&  -0.5&   0.2&  -0.2&  -0.9&   0.9&  -0.0&   0.6&   0.6&   0.2&  -1.6&   0.3&  -0.1&   0.5&   3.7&  -2.9&  -0.6&  -3.1&  -0.9&   1.5 \\ \hline
\hline
y&\frac{{\rm d}\sigma}{{\rm d}y}&\delta_{unc}&\delta_1&\delta_2&\delta_3&\delta_4&\delta_5&\delta_6&\delta_7&\delta_8&\delta_9&\delta_{10}&\delta_{11}&\delta_{12}&\delta_{13}&\delta_{14}&\delta_{15}&\delta_{16}&\delta_{17}&\delta_{18}&\delta_{19}&\delta_{20}&\delta_{21}&\delta_{22}&\delta_{br} \\
&$[\SI{}{nb}]$&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%] \\ \hline
0.02:0.05&  12.13&   5.8&  -0.6&   0.6&  -0.2&   0.8&   1.0&  -0.6&  -0.1&   1.4&   1.0&  -0.1&   0.0&  -2.3&  -0.2&   0.8&  -2.6&  -0.7&   5.4&   4.8&   2.7&   1.4&   0.4&  -0.6&   1.5 \\ 
0.05:0.09&  18.84&   3.9&  -1.3&   1.5&   0.2&   0.4&   1.0&   0.4&  -0.2&  -0.1&  -0.2&  -0.2&  -0.4&  -1.9&  -0.8&   0.1&   0.2&  -0.7&   1.6&   0.4&   2.2&  -0.7&   0.7&   0.2&   1.5 \\ 
0.09:0.13&  16.99&   3.4&  -1.3&   1.7&   0.2&   0.4&   0.8&   0.8&  -0.3&  -0.5&  -0.6&  -0.1&  -0.7&  -1.7&  -0.9&  -0.2&   0.4&  -0.9&   0.7&  -0.3&   1.9&  -0.7&  -0.1&   0.7&   1.5 \\ 
0.13:0.18&  13.35&   3.7&  -1.2&   1.3&   0.2&   0.4&   0.9&   0.7&  -0.4&   0.1&  -0.2&   0.0&  -0.6&  -1.9&  -0.7&   0.0&   0.4&  -0.4&  -0.5&   0.1&   1.4&  -1.8&  -0.0&   0.5&   1.5 \\ 
0.18:0.26&  11.19&   3.4&  -1.4&   1.5&   0.0&   0.5&   0.6&   0.9&  -0.4&  -0.2&  -0.5&   0.1&  -0.8&  -1.7&  -0.8&  -0.3&   0.2&  -0.5&  -0.2&  -0.2&   0.2&   0.6&  -0.2&   0.3&   1.5 \\
0.26:0.36&   7.649&   3.7&  -1.4&   1.5&   0.4&   0.2&   0.7&   1.0&  -0.5&  -0.1&  -0.5&   0.0&  -0.7&  -1.9&  -0.7&  -0.4&   1.0&  -1.0&  -0.5&  -1.0&   0.5&  -0.1&  -0.3&   0.4&   1.5 \\ 
0.36:0.50&   4.783&   4.0&  -1.7&   1.7&   0.6&   0.2&   0.7&   1.1&  -0.5&  -0.6&  -0.7&  -0.1&  -0.7&  -1.8&  -0.7&  -0.6&   2.1&  -0.2&  -0.4&  -2.4&   0.8&  -0.2&  -0.7&   0.7&   1.5 \\ 
0.50:0.70&   2.648&   5.6&  -2.2&   1.7&   0.9&  -0.4&   0.2&   0.8&  -0.4&  -0.4&  -1.0&  -0.6&  -0.5&  -2.1&  -0.5&  -0.8&   2.8&  -0.4&   0.3&  -2.8&  -1.4&   1.7&  -0.9&   0.3&   1.5 \\ \hline
\end{tabu}
%\end{center}
\caption[Combined \Dstar cross section with correlations as function of $p_T(\Dstar)$ and $\eta(\Dstar)$]
{The combined single-differential \Dstar cross sections as a function of $p_T(\Dstar)$ and $\eta(\Dstar)$, with their 
uncorrelated ($\delta_{unc}$), correlated ($\delta_1$ to $\delta_{22}$) and external branching-ratio ($\delta_{br}$) uncertainties.} 
\label{tab:comb:dstar:single:combinedfull1}
\end{table*}
%\end{sidewaystable}


==> content/combination/dstar/cs/combinedfull2.tex <==
%\begin{sidewaystable}[tbp]
\begin{table*}[tbp]
\footnotesize
%\begin{center}
\tabcolsep0.15mm
\renewcommand*{\arraystretch}{1.05}
\begin{tabu} to \textwidth{|>{$}c<{$}|>{$}l<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|} \hline
z(\Dstar)&\frac{{\rm d}\sigma}{{\rm d}z(\Dstar)}&\delta_{unc}&\delta_1&\delta_2&\delta_3&\delta_4&\delta_5&\delta_6&\delta_7&\delta_8&\delta_9&\delta_{10}&\delta_{11}&\delta_{12}&\delta_{13}&\delta_{14}&\delta_{15}&\delta_{16}&\delta_{17}&\delta_{18}&\delta_{19}&\delta_{20}&\delta_{21}&\delta_{22}&\delta_{br} \\ 
&$[\SI{}{nb}]$&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%] \\ \hline
0.000:0.100&   3.277&   9.5&   1.7&   1.9&  -0.0&   1.1&   0.5&  -1.0&   1.0&   0.5&  -0.9&   0.4&   0.2&   0.7&   0.1&   0.1&  -0.1&  -1.1&   3.4&  -2.0&   1.1&  -1.3&   0.7&   0.6&   1.5 \\ 
0.100:0.200&   7.346&   4.8&   1.8&   1.2&  -0.2&   1.1&   0.2&  -1.0&   0.8&   0.4&  -0.7&   0.1&   0.3&   0.7&   0.4&   0.1&   0.3&  -1.4&   2.5&  -1.5&   2.9&  -2.9&   0.9&   0.8&   1.5 \\ 
0.200:0.325&   8.612&   3.5&   2.0&   1.0&  -0.1&   0.9&   0.2&  -0.6&   0.6&   0.5&  -0.2&   0.1&   0.3&   0.5&   0.6&   0.1&   0.3&  -1.2&   2.0&   0.3&   0.9&  -2.0&   0.6&   0.5&   1.5 \\ 
0.325:0.450&   8.918&   2.7&   2.1&   1.0&  -0.1&   0.9&   0.2&  -0.4&   0.4&   0.5&  -0.0&   0.0&   0.4&   0.4&   0.6&  -0.0&   0.3&  -0.7&   1.6&   1.2&  -0.7&  -0.3&   0.0&   0.3&   1.5 \\ 
0.450:0.575&   8.827&   1.8&   2.3&   1.2&   0.0&   0.8&   0.4&  -0.0&   0.3&   0.5&   0.3&   0.0&   0.4&   0.3&   0.4&  -0.1&   0.3&  -0.4&   0.7&   1.6&   0.9&  -0.1&  -0.1&   0.8&   1.5 \\ 
0.575:0.800&   4.785&   2.4&   2.2&   1.4&   0.1&   0.9&   0.6&  -0.0&   0.6&   0.5&   0.2&   0.1&   0.6&   0.4&   0.1&  -0.1&   0.2&   0.8&  -0.5&   2.5&   2.5&   0.4&  -0.5&   0.7&   1.5 \\ 
0.800:1.000&   0.6308&   8.1&   1.6&   0.8&  -0.3&   2.4&   1.0&  -1.5&   1.5&   0.2&  -1.3&  -0.2&   1.3&   1.0&  -0.3&  -0.1&   0.9&   3.8&  -2.8&   3.8&   4.4&   4.0&   3.1&  -0.4&   1.5 \\ \hline
\hline
Q^2&\frac{{\rm d}\sigma}{{\rm d}Q^2}&\delta_{unc}&\delta_1&\delta_2&\delta_3&\delta_4&\delta_5&\delta_6&\delta_7&\delta_8&\delta_9&\delta_{10}&\delta_{11}&\delta_{12}&\delta_{13}&\delta_{14}&\delta_{15}&\delta_{16}&\delta_{17}&\delta_{18}&\delta_{19}&\delta_{20}&\delta_{21}&\delta_{22}&\delta_{br} \\
$[\SI{}{GeV^2}]$&$[\SI{}{nb/GeV^2}]$&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%] \\ \hline
   5:   8&   0.4735&   4.0&   1.4&  -1.4&  -0.9&   0.9&  -0.9&   0.6&  -0.9&  -0.3&   1.1&  -0.2&   0.9&  -1.3&   0.7&   0.7&   0.8&   1.5&  -1.0&  -0.6&   0.7&  -2.1&  -1.2&   0.3&   1.5 \\ 
   8:  10&   0.2964&   4.3&   1.2&  -1.3&  -0.7&   0.7&  -1.0&   0.8&  -0.6&  -0.4&   1.0&   0.0&   0.8&  -1.0&   0.7&   0.4&   1.1&   1.1&  -0.2&  -0.1&  -0.1&   0.5&  -0.5&  -0.1&   1.5 \\ 
  10:  13&   0.2117&   3.8&   0.8&  -1.9&  -0.8&   0.8&  -0.6&   0.8&  -0.5&  -0.6&   1.0&  -0.1&   0.6&  -0.6&   0.4&  -0.1&   0.9&   1.0&  -0.9&   0.7&  -0.3&  -1.2&  -0.5&   0.4&   1.5 \\ 
  13:  19&   0.1236&   3.2&   0.8&  -1.8&  -0.8&   0.8&  -0.7&   0.8&  -0.4&  -0.7&   1.0&  -0.1&   0.6&  -0.6&   0.6&   0.0&   0.8&   0.8&  -0.0&   0.0&  -1.0&  -0.9&  -0.3&   0.5&   1.5 \\
  19:  28&   0.07263&   3.5&   0.8&  -1.8&  -0.7&   0.7&  -0.7&   0.8&  -0.3&  -0.7&   0.9&  -0.1&   0.6&  -0.6&   0.5&   0.2&   0.7&   0.7&  -0.0&   0.2&  -0.9&  -0.6&  -0.3&   0.4&   1.5 \\ 
  28:  40&   0.03970&   3.7&   0.7&  -1.9&  -0.8&   0.8&  -0.6&   0.8&  -0.3&  -0.8&   1.0&  -0.2&   0.5&  -0.5&   0.3&   0.0&   0.8&   0.6&  -0.6&   0.5&  -0.7&  -1.7&  -0.3&   0.6&   1.5 \\ 
  40:  60&   0.01635&   4.4&   0.7&  -2.0&  -0.8&   0.8&  -0.5&   0.7&  -0.3&  -0.7&   0.8&  -0.3&   0.6&  -0.4&   0.6&  -0.4&   0.5&   0.9&   0.5&  -0.0&  -1.5&  -2.6&  -0.6&   0.7&   1.5 \\ 
  60: 100&   0.007445&   5.2&   0.8&  -1.9&  -0.8&   0.9&  -0.5&   0.7&  -0.4&  -0.6&   0.9&  -0.3&   0.6&  -0.4&   0.7&  -0.3&   0.1&   0.2&   0.2&   0.9&  -1.6&  -0.4&   0.3&  -0.0&   1.5 \\ 
 100: 158&   0.002081&   7.2&   0.1&  -2.3&  -0.4&  -0.6&  -0.8&   0.3&  -0.2&  -0.8&   1.0&   0.0&   0.6&  -0.0&  -0.4&  -1.3&   0.7&   0.8&  -1.6&   1.8&  -2.5&  -0.8&  -1.3&  -0.5&   1.5 \\ 
 158: 251&   0.0008817&   7.6&   0.3&  -1.8&  -0.5&  -0.4&  -0.9&   0.2&  -0.4&  -0.8&   1.1&  -0.0&   0.7&  -0.3&  -0.0&  -1.0&   1.1&   0.0&  -0.2&   2.1&  -2.1&  -0.8&  -2.0&  -0.6&   1.5 \\ 
 251:1000&   0.0000749&  11.4&  -0.1&  -2.3&  -0.6&  -0.4&  -0.5&   0.2&  -0.2&  -0.9&   0.9&  -0.0&   0.6&   0.6&   0.2&  -1.6&   0.3&  -0.1&   0.5&   3.7&  -2.9&  -0.6&  -3.1&  -0.9&   1.5 \\ \hline
\hline
y&\frac{{\rm d}\sigma}{{\rm d}y}&\delta_{unc}&\delta_1&\delta_2&\delta_3&\delta_4&\delta_5&\delta_6&\delta_7&\delta_8&\delta_9&\delta_{10}&\delta_{11}&\delta_{12}&\delta_{13}&\delta_{14}&\delta_{15}&\delta_{16}&\delta_{17}&\delta_{18}&\delta_{19}&\delta_{20}&\delta_{21}&\delta_{22}&\delta_{br} \\
&$[\SI{}{nb}]$&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%] \\ \hline
0.02:0.05&  12.13&   5.8&  -0.6&   0.6&  -0.2&   0.8&   1.0&  -0.6&  -0.1&   1.4&   1.0&  -0.1&   0.0&  -2.3&  -0.2&   0.8&  -2.6&  -0.7&   5.4&   4.8&   2.7&   1.4&   0.4&  -0.6&   1.5 \\ 
0.05:0.09&  18.84&   3.9&  -1.3&   1.5&   0.2&   0.4&   1.0&   0.4&  -0.2&  -0.1&  -0.2&  -0.2&  -0.4&  -1.9&  -0.8&   0.1&   0.2&  -0.7&   1.6&   0.4&   2.2&  -0.7&   0.7&   0.2&   1.5 \\ 
0.09:0.13&  16.99&   3.4&  -1.3&   1.7&   0.2&   0.4&   0.8&   0.8&  -0.3&  -0.5&  -0.6&  -0.1&  -0.7&  -1.7&  -0.9&  -0.2&   0.4&  -0.9&   0.7&  -0.3&   1.9&  -0.7&  -0.1&   0.7&   1.5 \\ 
0.13:0.18&  13.35&   3.7&  -1.2&   1.3&   0.2&   0.4&   0.9&   0.7&  -0.4&   0.1&  -0.2&   0.0&  -0.6&  -1.9&  -0.7&   0.0&   0.4&  -0.4&  -0.5&   0.1&   1.4&  -1.8&  -0.0&   0.5&   1.5 \\ 
0.18:0.26&  11.19&   3.4&  -1.4&   1.5&   0.0&   0.5&   0.6&   0.9&  -0.4&  -0.2&  -0.5&   0.1&  -0.8&  -1.7&  -0.8&  -0.3&   0.2&  -0.5&  -0.2&  -0.2&   0.2&   0.6&  -0.2&   0.3&   1.5 \\
0.26:0.36&   7.649&   3.7&  -1.4&   1.5&   0.4&   0.2&   0.7&   1.0&  -0.5&  -0.1&  -0.5&   0.0&  -0.7&  -1.9&  -0.7&  -0.4&   1.0&  -1.0&  -0.5&  -1.0&   0.5&  -0.1&  -0.3&   0.4&   1.5 \\ 
0.36:0.50&   4.783&   4.0&  -1.7&   1.7&   0.6&   0.2&   0.7&   1.1&  -0.5&  -0.6&  -0.7&  -0.1&  -0.7&  -1.8&  -0.7&  -0.6&   2.1&  -0.2&  -0.4&  -2.4&   0.8&  -0.2&  -0.7&   0.7&   1.5 \\ 
0.50:0.70&   2.648&   5.6&  -2.2&   1.7&   0.9&  -0.4&   0.2&   0.8&  -0.4&  -0.4&  -1.0&  -0.6&  -0.5&  -2.1&  -0.5&  -0.8&   2.8&  -0.4&   0.3&  -2.8&  -1.4&   1.7&  -0.9&   0.3&   1.5 \\ \hline
\end{tabu}
%\end{center}
\caption[Combined \Dstar cross section with correlations as function of $z(\Dstar)$, $Q^2$ and $y$]
{The combined single-differential \Dstar cross sections as a function of $z(\Dstar)$, $Q^2$ and $y$, with their 
uncorrelated ($\delta_{unc}$), correlated ($\delta_1$ to $\delta_{22}$) and external branching-ratio ($\delta_{br}$) uncertainties.} 
\label{tab:comb:dstar:single:combinedfull2}
\end{table*}
%\end{sidewaystable}


==> content/combination/dstar/input/set_h1hera2_q2y.tex <==
\begin{sidewaystable}[tbp]
\footnotesize
%\begin{center}
\tabcolsep1.2mm
\renewcommand*{\arraystretch}{0.96}
\begin{tabu}{|>{$}c<{$}|>{$}c<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|} \hline
\multicolumn{20}{|c|}{H1 HERA-II (datasets I+II)}\\ \hline
Q^2&y&\frac{{\rm d}^2\sigma}{{\rm d}Q^2{\rm d}y}&%\multicolumn{17}{c|}{$\delta$}\\ \cline{4-20}
\delta_{stat}&\delta_{uncor}&\delta_{1}&\delta_{2}&\delta_{3}&\delta_{4}&\delta_{5}&\delta_{6}&\delta_{7}&\delta_{8}&\delta_{9}&\delta_{10}&\delta_{24}&\delta_{25}&\delta_{26}&\delta_{27}&\delta_{28}\\ \hline
[$\SI{}{GeV^2}$]&&[$\SI{}{nb/GeV^2}]$&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]\\ \hline
   5.5:   9.0&  0.02:0.05&   0.122771&    11.7&    5.0&    2.9&    3.2&    1.0&   -1.8&    1.7&   -0.5&   -0.0&   -4.6&   -1.3&   -0.9&    0.0&   -0.2&    0.1&    0.1&   -0.2\\
   5.5:   9.0&  0.05:0.09&   0.208477&     7.6&    5.0&    2.9&    3.2&    1.0&   -2.8&    1.6&   -0.7&   -0.0&   -4.0&   -2.3&   -1.7&    0.3&    0.1&   -0.1&    0.1&   -0.2\\
   5.5:   9.0&  0.09:0.16&   0.321166&     5.6&    5.0&    2.9&    3.2&    1.0&   -1.7&    4.4&   -0.3&   -0.0&   -1.3&   -2.7&   -4.0&   -0.0&    0.4&   -0.1&    0.1&   -0.2\\
   5.5:   9.0&  0.16:0.32&   0.447618&     4.7&    5.0&    2.9&    3.2&    1.0&   -1.6&    3.4&   -0.4&   -0.0&   -3.4&   -2.5&   -4.8&    0.1&    0.1&    0.0&    0.1&   -0.2\\
   5.5:   9.0&  0.32:0.70&   0.307615&     7.2&    5.0&    2.9&    3.2&    1.0&    3.1&    3.7&   -0.3&   -0.0&    1.5&   -2.8&   -6.4&    0.3&    0.1&    0.1&    0.1&   -0.2\\
   9.0:  14.0&  0.02:0.05&   0.068712&    18.0&    5.0&    2.9&    3.2&    1.0&   -3.7&    4.3&   -1.2&   -0.0&   -4.1&    0.9&    3.5&   -0.0&   -0.0&   -0.0&    0.0&   -0.0\\
   9.0:  14.0&  0.05:0.09&   0.149424&     9.1&    5.0&    2.9&    3.2&    1.0&   -3.3&    3.6&   -0.3&   -0.0&   -4.3&   -2.5&   -2.9&   -0.0&   -0.0&   -0.0&    0.0&   -0.0\\
   9.0:  14.0&  0.09:0.16&   0.203839&     7.6&    5.0&    2.9&    3.2&    1.0&   -1.9&    3.1&   -0.1&   -0.0&   -2.8&   -2.5&   -3.0&   -0.0&   -0.0&   -0.0&    0.0&   -0.0\\
   9.0:  14.0&  0.16:0.32&   0.331893&     6.7&    5.0&    2.9&    3.2&    1.0&    1.8&    1.9&    0.3&   -0.0&   -1.1&   -2.3&   -3.0&   -0.0&   -0.0&   -0.0&    0.0&   -0.0\\
   9.0:  14.0&  0.32:0.70&   0.273543&     7.7&    5.0&    2.9&    3.2&    1.0&    2.9&    2.5&    0.1&   -0.0&    1.2&   -2.8&   -5.3&   -0.0&   -0.0&   -0.0&    0.0&   -0.0\\
  14.0:  23.0&  0.02:0.05&   0.067376&   13.0&    5.0&    2.9&    3.2&    1.0&   -5.0&   -0.8&   -1.2&   -0.0&   -1.9&   -1.5&    3.5&   -0.0&   -0.0&   -0.0&    0.0&   -0.0\\
  14.0:  23.0&  0.05:0.09&   0.129681&     9.8&    5.0&    2.9&    3.2&    1.0&   -1.7&    2.7&   -0.8&   -0.0&   -4.3&   -2.0&   -2.1&   -0.0&   -0.0&   -0.0&    0.0&   -0.0\\
  14.0:  23.0&  0.09:0.16&   0.191319&     7.0&    5.0&    2.9&    3.2&    1.0&   -2.1&    2.0&   -0.8&   -0.0&   -6.4&   -2.4&   -3.1&   -0.0&   -0.0&   -0.0&    0.0&   -0.0\\
  14.0:  23.0&  0.16:0.32&   0.301013&     5.8&    5.0&    2.9&    3.2&    1.0&    1.7&    3.1&    0.6&   -0.0&   -1.4&   -2.6&   -3.2&   -0.0&   -0.0&   -0.0&    0.0&   -0.0\\
  14.0:  23.0&  0.32:0.70&   0.225959&     8.4&    5.0&    2.9&    3.2&    1.0&    2.7&    3.1&    0.3&   -0.0&    4.3&   -2.9&   -5.4&   -0.0&   -0.0&   -0.0&    0.0&   -0.0\\
  23.0:  45.0&  0.02:0.05&   0.057502&   13.3&    5.0&    2.9&    3.2&    1.0&   -5.7&    1.9&   -3.1&   -0.0&  -12.9&    0.7&    1.8&   -0.0&   -0.0&   -0.0&    0.0&   -0.0\\
  23.0:  45.0&  0.05:0.09&   0.105608&    10.8&    5.0&    2.9&    3.2&    1.0&   -2.5&    3.0&   -1.0&   -0.0&   -5.0&   -2.4&   -2.1&   -0.0&   -0.0&   -0.0&    0.0&   -0.0\\
  23.0:  45.0&  0.09:0.16&   0.186974&     7.8&    5.0&    2.9&    3.2&    1.0&   -2.9&    3.0&   -0.1&   -0.0&   -4.7&   -2.5&   -2.5&   -0.0&   -0.0&   -0.0&    0.0&   -0.0\\
  23.0:  45.0&  0.16:0.32&   0.262564&     6.2&    5.0&    2.9&    3.2&    1.0&    2.0&    2.5&    0.4&   -0.0&   -1.8&   -2.5&   -2.6&   -0.0&   -0.0&   -0.0&    0.0&   -0.0\\
  23.0:  45.0&  0.32:0.70&   0.254796&     7.9&    5.0&    2.9&    3.2&    1.0&    2.7&    2.2&    0.4&   -0.0&    3.2&   -2.9&   -4.7&   -0.0&   -0.0&   -0.0&    0.0&   -0.0\\
  45.0: 100.0&  0.02:0.05&   0.008933&  47.8&    5.0&    2.9&    3.2&    1.0&   -9.7&   -0.5&   -2.4&   -0.0&   -3.6&    0.9&    2.9&   -0.0&   -0.0&   -0.0&    0.0&   -0.0\\
  45.0: 100.0&  0.05:0.09&   0.054921&   16.6&    5.0&    2.9&    3.2&    1.0&   -4.8&    2.6&   -0.5&   -0.0&   -4.9&   -1.9&   -0.6&   -0.0&   -0.0&   -0.0&    0.0&   -0.0\\
  45.0: 100.0&  0.09:0.16&   0.082987&   13.1&    5.0&    2.9&    3.2&    1.0&   -1.5&    2.3&   -0.6&   -0.0&   -7.2&   -2.1&   -4.1&   -0.0&   -0.0&   -0.0&    0.0&   -0.0\\
  45.0: 100.0&  0.16:0.32&   0.208217&     7.9&    5.0&    2.9&    3.2&    1.0&   -2.4&    2.5&    0.5&   -0.0&   -4.7&   -3.2&   -4.6&   -0.0&   -0.0&   -0.0&    0.0&   -0.0\\
  45.0: 100.0&  0.32:0.70&   0.152967&    11.7&    5.0&    2.9&    3.2&    1.0&    3.1&    2.7&    0.2&   -0.0&    4.8&   -2.2&   -2.8&   -0.0&   -0.0&   -0.0&    0.0&   -0.0\\
 100.0: 158.0&  0.02:0.32&   0.060493&   14.0&    6.1&    6.9&    3.2&    0.0&    5.2&    6.8&    0.5&    0.2&    4.7&    0.0&    0.0&   -0.2&   -0.2&    0.0&    0.0&   -0.0\\
 100.0: 158.0&  0.32:0.70&   0.049052&   15.0&    6.1&    6.9&    3.2&    0.0&    1.4&    0.7&    1.8&    0.6&    0.9&    0.0&    0.0&   -0.1&   -0.1&   -0.1&    0.0&   -0.1\\
 158.0: 251.0&  0.02:0.30&   0.042029&   13.0&    6.7&    6.9&    3.2&    0.0&    2.2&    0.5&    1.2&    0.4&    4.5&    0.0&    0.0&   -0.0&   -0.0&   -0.0&    0.0&   -0.0\\
 158.0: 251.0&  0.30:0.70&   0.030206&   15.0&    6.7&    6.9&    3.2&    0.0&    1.0&    1.8&    1.7&    0.7&    3.6&   -0.0&    0.0&   -0.0&   -0.0&   -0.0&    0.0&   -0.0\\
 251.0:1000.0&  0.02:0.26&   0.016264&   25.0&    8.4&    6.9&    3.2&    0.0&    3.7&    1.7&    1.5&    0.2&    7.4&    0.0&   -0.0&   -0.3&   -0.3&   -0.1&    0.1&    0.1\\
 251.0:1000.0&  0.26:0.70&   0.027092&   20.0&    8.4&    6.9&    3.2&    0.0&    0.2&    1.0&    1.6&    0.6&    7.2&   -0.0&   -0.0&   -0.1&   -0.1&    0.1&    0.1&   -0.1\\
\hline
\end{tabu}
%\end{center}
\caption[Input H1 HERA-II double-differential \Dstar cross section]
{Input data H1 HERA-II (datasets I+II) used for the combination of the \Dstar double-differential cross section as a function of $Q^2$ and $y$. 
The table reports for each bin the input differential cross section ($\frac{{\rm d}^2\sigma}{{\rm d}Q^2{\rm d}y}$) together with its statistical ($\delta_{stat}$), 
uncorrelated ($\delta_{uncor}$) and all correlated (all other $\delta_{...}$)
%, $XXX \neq stat$, $XXX \neq uncor$) 
uncertainties.}
\label{tab:comb:dstar:single:inputq2yh1hera2}
\end{sidewaystable}


==> content/combination/dstar/input/set_h1zeus_eta.tex <==
\begin{sidewaystable}[tbp]
\small
%\begin{center}
\tabcolsep1.2mm
\renewcommand*{\arraystretch}{0.97}
\begin{tabu}{|>{$}c<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|} \hline
\multicolumn{16}{|c|}{H1 HERA-II (datasets I+II)}\\ \hline
\eta(\Dstar)&{\rm d}\sigma/{\rm d}\eta(\Dstar)&%\multicolumn{14}{c|}{$\delta$}\\ \cline{3-16}
\delta_{stat}&\delta_{uncor}&\delta_{1}&\delta_{2}&\delta_{3}&\delta_{4}&\delta_{5}&\delta_{6}&\delta_{7}&\delta_{8}&\delta_{9}&\delta_{10}&\delta_{sw}&\delta_{11}\\ \hline
&[$\SI{}{nb}]$&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]\\ \hline
-1.50:-1.25&   1.264195&    6.3&    5.0&    2.9&    3.2&    1.0&   -0.6&    1.2&    0.0&   -0.0&   -1.0&   -1.2&   -1.6&    0.2&    0.3\\
-1.25:-1.00&   1.369066&    4.7&    5.0&    2.9&    3.2&    1.0&   -0.4&    1.1&   -0.0&   -0.0&    0.1&   -1.2&   -2.3&    0.2&    0.5\\
-1.00:-0.75&   1.564379&    4.1&    5.0&    2.9&    3.2&    1.0&   -0.4&    1.1&   -0.0&   -0.0&    0.2&   -1.2&   -2.6&    0.2&    0.5\\
-0.75:-0.50&   1.711417&    4.0&    5.0&    2.9&    3.2&    1.0&   -0.3&    1.0&   -0.0&   -0.0&   -0.5&   -1.1&   -1.6&    0.1&    0.6\\
-0.50:-0.25&   1.654022&    4.0&    5.0&    2.9&    3.2&    1.0&   -0.3&    0.9&   -0.0&   -0.0&   -0.1&   -1.0&   -1.4&    0.2&    0.7\\
-0.25: 0.00&   1.719374&    4.0&    5.0&    2.9&    3.2&    1.0&   -0.2&    0.9&   -0.0&   -0.0&   -1.0&   -1.1&   -1.7&    0.1&    0.7\\
 0.00: 0.25&   1.761646&    4.2&    5.0&    2.9&    3.2&    1.0&   -0.2&    0.9&   -0.0&   -0.0&   -0.7&   -0.7&   -0.9&    0.1&    0.7\\
 0.25: 0.50&   1.773855&    4.4&    5.0&    2.9&    3.2&    1.0&   -0.2&    0.8&   -0.0&   -0.0&   -1.0&   -0.7&   -1.7&    0.1&    0.7\\
 0.50: 0.75&   1.851288&    4.4&    5.0&    2.9&    3.2&    1.0&   -0.2&    0.9&    0.0&   -0.0&   -0.7&   -0.8&   -1.6&    0.2&    0.7\\
 0.75: 1.00&   1.838827&    4.6&    5.0&    2.9&    3.2&    1.0&   -0.2&    0.8&    0.0&   -0.0&   -1.3&   -1.1&   -2.4&    0.1&    0.6\\
 1.00: 1.25&   2.112178&    4.7&    5.0&    2.9&    3.2&    1.0&   -0.2&    0.8&   -0.0&   -0.0&   -1.3&   -0.9&   -2.2&    0.2&    0.5\\
 1.25: 1.50&   1.808955&    7.1&    5.0&    2.9&    3.2&    1.0&   -0.2&    0.9&   -0.0&   -0.0&    0.1&   -1.1&   -2.3&    0.2&    0.6\\
\hline
\end{tabu}

\begin{tabu}{|>{$}c<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|} \hline
\multicolumn{15}{|c|}{ZEUS HERA-II (datasets III)}\\ \hline
\eta(\Dstar)&{\rm d}\sigma/{\rm d}\eta(\Dstar)&%\multicolumn{13}{c|}{$\delta$}\\ \cline{3-15}
\delta_{stat}&\delta_{uncor}&\delta_{12}&\delta_{13}&\delta_{14}&\delta_{15}&\delta_{16}&\delta_{17}&\delta_{18}&\delta_{19}&\delta_{20}&\delta_{21}&\delta_{22}\\ \hline
&[$\SI{}{nb}]$&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]\\ \hline
-1.50:-1.25&   1.480000&    7.5&    3.5&    1.7&    1.8&   -1.4&   -0.2&    1.3&    0.1&   -0.0&    2.1&    4.8&    2.5&    1.9\\
-1.25:-1.00&   1.660000&    5.4&    2.8&    2.3&    0.5&   -0.9&   -0.3&    1.0&   -0.0&    0.2&    2.0&    3.8&    1.2&    1.9\\
-1.00:-0.75&   1.610000&    4.9&    4.1&    3.8&    0.8&   -0.7&   -0.3&    1.0&    0.1&   -0.0&    1.9&    3.2&    0.6&    1.9\\
-0.75:-0.50&   1.850000&    4.2&    2.1&    1.5&    0.9&   -0.6&   -0.2&    0.7&   -0.1&    0.0&    1.9&    2.7&    0.7&    1.9\\
-0.50:-0.25&   1.940000&    4.2&    1.9&   -0.6&    1.0&   -0.5&   -0.1&    0.6&   -0.1&    0.2&    1.8&    2.4&    0.7&    1.9\\
-0.25: 0.00&   2.020000&    4.0&    2.2&    3.8&    0.9&   -0.3&   -0.0&    0.6&   -0.0&    0.3&    1.8&    2.3&    1.1&    1.9\\
 0.00: 0.25&   1.900000&    4.4&    2.3&   -2.5&    0.7&   -0.4&   -0.2&    0.5&    0.1&   -0.1&    1.8&    2.2&    1.1&    1.9\\
 0.25: 0.50&   1.970000&    4.4&    2.0&    3.5&    0.3&   -0.3&   -0.1&    0.4&    0.1&    0.2&    1.8&    2.4&    1.0&    1.9\\
 0.50: 0.75&   1.960000&    4.7&    2.2&    2.3&    0.8&   -0.3&   -0.1&    0.4&    0.1&    0.1&    1.8&    2.7&    0.5&    1.9\\
 0.75: 1.00&   2.000000&    4.9&    2.3&    4.1&    0.8&   -0.2&   -0.1&    0.3&    0.1&   -0.5&    1.8&    3.2&    0.6&    1.9\\
 1.00: 1.25&   2.000000&    5.8&    2.9&   -3.6&    0.9&   -0.5&   -0.1&    0.4&   -0.0&    0.1&    1.8&    3.8&    0.3&    1.9\\
 1.25: 1.50&   1.840000&    7.7&    4.8&    7.8&    1.1&   -0.1&   -0.0&    0.4&    0.0&   -0.6&    1.9&    4.7&    0.1&    1.9\\
\hline
\end{tabu}
%\end{center}
\caption[Input single-differential \Dstar cross section as function of $\eta(\Dstar)$]
{Input data used for the combination of the \Dstar single-differential cross section as a function of $\eta(\Dstar)$. 
The tables report for each bin the input differential cross section (${\rm d}\sigma/{\rm d}\eta(\Dstar)$) together with its statistical ($\delta_{stat}$), 
uncorrelated ($\delta_{uncor}$) and all correlated (all other $\delta_{...}$)
%, $XXX \neq stat$, $XXX \neq uncor$) 
uncertainties; the theoretical uncertainties from the swimming procedure are shown separately ($\delta_{sw}$).}
\label{tab:comb:dstar:single:inputeta}
\end{sidewaystable}


==> content/combination/dstar/input/set_h1zeus_pt.tex <==
\begin{sidewaystable}[tbp]
\small
%\begin{center}
\tabcolsep1.2mm
\renewcommand*{\arraystretch}{1.03}
%\begin{tabu}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|} \hline
\begin{tabu}{|>{$}c<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|} \hline
\multicolumn{16}{|c|}{H1 HERA-II (datasets I+II)}\\ \hline
p_T(\Dstar)&{\rm d}\sigma/{\rm d}p_T(\Dstar)&%\multicolumn{14}{c|}{$\delta$}\\ \cline{3-16}
\delta_{stat}&\delta_{uncor}&\delta_{1}&\delta_{2}&\delta_{3}&\delta_{4}&\delta_{5}&\delta_{6}&\delta_{7}&\delta_{8}&\delta_{9}&\delta_{10}&\delta_{sw}&\delta_{11}\\ \hline
[$\SI{}{GeV}$]&[$\SI{}{nb/GeV}]$&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]\\ \hline
 1.50: 1.88&   2.370403&    6.5&    5.0&    2.9&    3.2&    1.0&   -0.5&    1.5&    0.0&   -0.0&   -1.2&    0.3&    1.2&    0.1&    0.1\\
 1.88: 2.28&   2.072862&    4.6&    5.0&    2.9&    3.2&    1.0&   -0.3&    1.4&   -0.0&   -0.0&   -0.9&   -0.2&    0.6&    0.1&    0.2\\
 2.28: 2.68&   1.990029&    3.6&    5.0&    2.9&    3.2&    1.0&   -0.3&    1.2&    0.0&   -0.0&   -1.7&   -0.2&    0.2&    0.1&    0.2\\
 2.68: 3.08&   1.414324&    3.6&    5.0&    2.9&    3.2&    1.0&   -0.2&    1.1&   -0.0&   -0.0&   -0.8&   -0.2&    0.5&    0.2&    0.3\\
 3.08: 3.50&   1.181779&    3.7&    5.0&    2.9&    3.2&    1.0&   -0.2&    0.9&    0.0&   -0.0&   -0.5&   -0.1&    0.5&    0.2&    0.3\\
 3.50: 4.00&   0.843302&    3.5&    5.0&    2.9&    3.2&    1.0&   -0.2&    0.7&   -0.0&   -0.0&   -0.7&   -0.1&    0.5&    0.3&    0.4\\
 4.00: 4.75&   0.603741&    3.1&    5.0&    2.9&    3.2&    1.0&   -0.1&    0.5&   -0.0&   -0.0&   -0.8&   -0.3&   -0.3&    0.3&    0.6\\
 4.75: 6.00&   0.299299&    3.2&    5.0&    2.9&    3.2&    1.0&   -0.1&    0.3&    0.0&   -0.0&   -0.7&   -0.3&   -1.0&    0.4&    1.2\\
 6.00: 8.00&   0.109185&    4.4&    5.0&    2.9&    3.2&    1.0&    0.1&    0.1&    0.0&   -0.0&   -0.1&   -0.4&   -0.6&    1.2&    3.0\\
 8.00:11.00&   0.033956&    7.1&    5.0&    2.9&    3.2&    1.0&    0.1&    0.2&   -0.0&   -0.0&   -2.9&   -0.4&   -2.9&    4.0&    5.1\\
11.00:20.00&   0.003892&   15.8&    5.0&    2.9&    3.2&    1.0&    0.1&   -0.1&    0.0&   -0.0&   -0.6&   -0.7&   -3.2&    5.6&    7.3\\
\hline
\end{tabu}

\begin{tabu}{|>{$}c<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|} \hline
\multicolumn{15}{|c|}{ZEUS HERA-II (datasets III)}\\ \hline
p_T(\Dstar)&{\rm d}\sigma/{\rm d}p_T(\Dstar)&%\multicolumn{13}{c|}{$\delta$}\\ \cline{3-15}
\delta_{stat}&\delta_{uncor}&\delta_{12}&\delta_{13}&\delta_{14}&\delta_{15}&\delta_{16}&\delta_{17}&\delta_{18}&\delta_{19}&\delta_{20}&\delta_{21}&\delta_{22}\\ \hline
[$\SI{}{GeV}$]&[$\SI{}{nb/GeV}]$&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]\\ \hline
 1.50: 1.88&   2.160000&    9.9&    4.5&   11.1&    0.7&   -0.9&   -0.2&    1.2&   -0.8&   -0.3&    3.4&    3.0&    1.4&    1.9\\
 1.88: 2.28&   2.300000&    5.8&    3.9&    7.4&    0.2&   -0.6&   -0.2&    0.8&   -1.0&   -0.4&    2.9&    3.0&    1.3&    1.9\\
 2.28: 2.68&   1.950000&    4.4&    1.8&    5.0&    0.2&   -0.5&   -0.2&    0.7&   -0.5&    0.1&    2.4&    3.0&    1.4&    1.9\\
 2.68: 3.08&   1.630000&    4.0&    1.2&    2.6&   -0.6&   -0.4&   -0.1&    0.5&    0.3&   -0.3&    2.0&    3.0&    1.5&    1.9\\
 3.08: 3.50&   1.220000&    3.8&    2.4&    1.9&   -0.0&   -0.3&   -0.1&    0.5&    0.2&   -0.1&    1.6&    3.0&    1.4&    1.9\\
 3.50: 4.00&   0.970000&    3.4&    1.5&    2.1&    0.0&   -0.3&   -0.1&    0.3&    0.5&    0.1&    1.4&    2.9&    1.2&    1.9\\
 4.00: 4.75&   0.630000&    3.2&    1.1&   -1.3&   -0.3&   -0.4&   -0.1&    0.6&    0.6&    0.1&    1.3&    2.9&    1.1&    1.9\\
 4.75: 6.00&   0.330000&    3.0&    1.8&    1.1&   -0.1&   -0.4&   -0.1&    0.3&    0.6&    0.2&    1.1&    2.8&    1.2&    1.9\\
 6.00: 8.00&   0.120000&    3.8&    2.3&   -3.3&   -0.0&   -0.3&   -0.2&    0.4&    0.4&    0.4&    1.1&    2.7&    1.3&    1.9\\
 8.00:11.00&   0.033000&    6.0&    2.4&    2.3&    0.7&   -0.3&   -0.1&    0.5&    0.3&    0.2&    1.0&    2.7&    0.7&    1.9\\
11.00:20.00&   0.003600&   12.3&    5.1&   13.5&    1.3&    0.3&    0.0&    0.3&    0.5&    0.2&    1.0&    2.6&    0.4&    1.9\\
\hline
\end{tabu}
%\end{center}
\caption[Input single-differential \Dstar cross section as function of $p_T(\Dstar)$]
{Input data used for the combination of the \Dstar single-differential cross section as a function of $p_T(\Dstar)$. 
The tables report for each bin the input differential cross section (${\rm d}\sigma/{\rm d}p_T(\Dstar)$) together with its statistical ($\delta_{stat}$), 
uncorrelated ($\delta_{uncor}$) and all correlated (all other $\delta_{...}$) uncertainties; the theoretical uncertainties from the swimming procedure are shown separately ($\delta_{sw}$).}
%, $XXX \neq stat$, $XXX \neq uncor$) 
%uncertainties.}
\label{tab:comb:dstar:single:inputpt}
\end{sidewaystable}


==> content/combination/dstar/input/set_h1zeus_q2.tex <==
\begin{sidewaystable}[tbp]
\small
%\begin{center}
\tabcolsep1.2mm
\renewcommand*{\arraystretch}{1.06}
\begin{tabu}{|>{$}c<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|} \hline
\multicolumn{14}{|c|}{H1 HERA-II (datasets I+II)}\\ \hline
Q^2&{\rm d}\sigma/{\rm d}Q^2&%\multicolumn{12}{c|}{$\delta$}\\ \cline{3-14}
\delta_{stat}&\delta_{uncor}&\delta_{1}&\delta_{2}&\delta_{3}&\delta_{4}&\delta_{5}&\delta_{6}&\delta_{7}&\delta_{8}&\delta_{9}&\delta_{10}\\ \hline
[$\SI{}{GeV^2}$]&[$\SI{}{nb/GeV^2}]$&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]\\ \hline
   5:   8&   0.450491&    3.4&    5.0&    2.9&    3.2&    1.0&   -0.1&    1.4&   -0.0&   -0.0&   -2.3&   -1.1&   -3.0\\
   8:  10&   0.278716&    4.8&    5.0&    2.9&    3.2&    1.0&   -0.1&    0.4&   -0.0&   -0.0&   -1.2&   -1.0&   -2.3\\
  10:  13&   0.198811&    4.4&    5.0&    2.9&    3.2&    1.0&   -0.2&    1.5&    0.0&   -0.0&   -0.4&   -1.2&   -1.5\\
  13:  19&   0.123919&    3.4&    5.0&    2.9&    3.2&    1.0&   -0.3&    1.2&   -0.0&   -0.0&   -0.6&   -1.0&   -1.3\\
  19:  28&   0.068075&    4.1&    5.0&    2.9&    3.2&    1.0&   -0.3&    0.9&    0.0&   -0.0&   -0.1&   -0.9&   -1.3\\
  28:  40&   0.037496&    4.4&    5.0&    2.9&    3.2&    1.0&   -0.5&    1.2&   -0.0&   -0.0&   -0.9&   -1.0&   -0.8\\
  40:  60&   0.015640&    6.1&    5.0&    2.9&    3.2&    1.0&   -0.6&    1.1&    0.0&   -0.0&    1.0&   -0.8&   -1.6\\
  60: 100&   0.007259&    6.2&    5.0&    2.9&    3.2&    1.0&   -0.7&    0.9&   -0.0&   -0.0&    0.9&   -1.0&   -1.8\\
 100: 158&   0.001862&   10.3&    4.4&    6.9&    3.2&    0.0&    3.3&    4.1&    1.0&    0.4&    3.2&    0.0&    0.0\\
 158: 251&   0.000777&    9.8&    4.8&    6.9&    3.2&    0.0&    1.7&    1.0&    1.3&    0.5&    4.1&    0.0&    0.0\\
 251:1000&   0.000058&   15.6&    6.0&    6.9&    3.2&    0.0&    1.5&    1.3&    1.4&    0.4&    7.3&    0.0&    0.0\\
\hline
\end{tabu}

\begin{tabu}{|>{$}c<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|} \hline
\multicolumn{15}{|c|}{ZEUS HERA-II (datasets III)}\\ \hline
Q^2&{\rm d}\sigma/{\rm d}Q^2&%\multicolumn{13}{c|}{$\delta$}\\ \cline{3-15}
\delta_{stat}&\delta_{uncor}&\delta_{12}&\delta_{13}&\delta_{14}&\delta_{15}&\delta_{16}&\delta_{17}&\delta_{18}&\delta_{19}&\delta_{20}&\delta_{21}&\delta_{22}\\ \hline
[$\SI{}{GeV^2}$]&[$\SI{}{nb/GeV^2}]$&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]\\ \hline
  5:   8&   0.499000&    3.9&    3.5&    5.5   & 0.9&    3.2&    0.8&    1.2&   -0.6&   -0.1&    2.1&    3.0&    1.6&    1.9\\
   8:  10&   0.307000&    4.3&    3.5&   -0.6  &  1.5&    1.1&    0.4&    0.6&   -1.0&   -0.1&    2.1&    3.0&    1.2&    1.9\\
  10:  13&   0.222000&    4.0&    2.2&    3.3  &  0.4&   -0.7&   -0.3&    0.5&   -0.9&   -0.1&    2.1&    3.0&    1.1&    1.9\\
  13:  19&   0.125000&    3.5&    1.5 &   2.2  &  1.0&   -0.9&   -0.1&    0.5&    0.9&    0.1&    2.0&    3.0&    1.1&    1.9\\
  19:  28&   0.075200&    3.7&    1.9 &   1.6 &   0.6&   -0.7&    0.2&    0.5&    0.6&    0.1&    1.9&    2.9&    1.0&    1.9\\
  28:  40&   0.041500&    3.9&    1.8  &  3.9 &   0.1 &  -1.2&   -0.1&    0.5&    0.2&    0.1&    1.7&    2.9&    1.1&    1.9\\
  40:  60&   0.016900&    4.7&    2.2   & 5.2 &   1.2  & -1.4&   -0.3&    0.4&    2.6&    0.4&    1.6&    2.9&    1.0&    1.9\\
  60: 100&   0.007470&    5.0&    4.8   & 0.4&   -0.4  & -2.8&   -1.2&    0.2&    1.5&    0.5&    1.5&    2.9&    1.4&    1.9\\
 100: 158&   0.002160&    9.1&    3.9    &2.0&    0.0   &-3.7&   -0.8&    0.3&   -1.3&    1.2&    1.3&    1.4&    0.9&    1.9\\
 158: 251&   0.000937&   10.8&    2.8    &2.0 &   0.6  & -2.2&   -0.7&    0.5&   -0.9&    0.9&    1.3&    1.3&    1.3&    1.9\\
 251:1000&   0.000100&   15.9&    4.5    &2.0&   -0.7  & -4.6&   -1.8&    0.9&   -0.6&    0.6&    1.3&    1.4&    0.4&    1.9\\
\hline
\end{tabu}
%\end{center}
\caption[Input single-differential \Dstar cross section as function of $Q^2$]
{Input data used for the combination of the \Dstar single-differential cross section as a function of $Q^2$. 
The tables report for each bin the input differential cross section (${\rm d}\sigma/{\rm d}Q^2$) together with its statistical ($\delta_{stat}$), 
uncorrelated ($\delta_{uncor}$) and all correlated (all other $\delta_{...}$)
%, $XXX \neq stat$, $XXX \neq uncor$) 
uncertainties.}
\label{tab:comb:dstar:single:inputq2}
\end{sidewaystable}


==> content/combination/dstar/input/set_h1zeus_y.tex <==
\begin{sidewaystable}[tbp]
\small
%\begin{center}
\tabcolsep1.2mm
\renewcommand*{\arraystretch}{1.1}
\begin{tabu}{|>{$}c<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|} \hline
\multicolumn{16}{|c|}{H1 HERA-II (datasets I+II)}\\ \hline
y&{\rm d}\sigma/{\rm d}y&%\multicolumn{14}{c|}{$\delta$}\\ \cline{3-16}
\delta_{stat}&\delta_{uncor}&\delta_{1}&\delta_{2}&\delta_{3}&\delta_{4}&\delta_{5}&\delta_{6}&\delta_{7}&\delta_{8}&\delta_{9}&\delta_{10}&\delta_{sw}&\delta_{11}\\ \hline
&[$\SI{}{nb}]$&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]\\ \hline
0.02:0.05&  12.304402&    5.2&    5.0&    2.9&    3.2&    1.0&   -3.9&    0.5&    7.0&   -0.0&   -5.6&   -1.3&    3.2&    0.1&    0.1\\
0.05:0.09&  16.866968&    4.2&    5.0&    2.9&    3.2&    1.0&   -1.1&    1.0&    1.4&   -0.0&   -1.3&   -0.9&   -1.9&    0.1&    0.3\\
0.09:0.13&  16.486118&    4.5&    5.0&    2.9&    3.2&    1.0&   -1.0&    1.0&    1.2&   -0.0&   -3.2&   -1.0&   -2.4&    0.1&    0.5\\
0.13:0.18&  13.279848&    4.8&    5.0&    2.9&    3.2&    1.0&   -0.4&    1.0&   -0.4&   -0.0&   -1.0&   -1.1&   -1.8&    0.1&    0.5\\
0.18:0.26&  11.401967&    3.9&    5.0&    2.9&    3.2&    1.0&    0.0&    1.0&   -0.8&   -0.0&   -2.1&   -0.8&   -2.5&    0.0&    0.6\\
0.26:0.36&   7.258390&    4.6&    5.0&    2.9&    3.2&    1.0&    0.5&    0.9&   -1.7&   -0.0&    0.0&   -1.2&   -2.9&    0.1&    0.7\\
0.36:0.50&   4.549839&    5.1&    5.0&    2.9&    3.2&    1.0&    1.0&    0.9&   -2.3&   -0.0&    1.5&   -1.0&   -4.2&    0.1&    0.9\\
0.50:0.70&   2.324644&    8.1&    5.0&    2.9&    3.2&    1.0&    1.6&    0.7&    0.2&   -0.0&    4.2&   -1.0&   -4.6&    0.2&    1.1\\
\hline
\end{tabu}

\begin{tabu}{|>{$}c<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|} \hline
\multicolumn{15}{|c|}{ZEUS HERA-II (datasets III)}\\ \hline
y&{\rm d}\sigma/{\rm d}y&%\multicolumn{13}{c|}{$\delta$}\\ \cline{3-15}
\delta_{stat}&\delta_{uncor}&\delta_{12}&\delta_{13}&\delta_{14}&\delta_{15}&\delta_{16}&\delta_{17}&\delta_{18}&\delta_{19}&\delta_{20}&\delta_{21}&\delta_{22}\\ \hline
&[$\SI{}{nb}]$&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]\\ \hline
0.02:0.05&  12.000000&    7.9&    5.5&   -7.8&   -5.9&   -7.1&   10.9&   -0.0&    0.3&    0.0&    2.1&    4.2&    1.9&    1.9\\
0.05:0.09&  20.700000&    3.4&    3.3&    2.3&   -0.8&   -2.2&    4.0&    0.0&    0.0&   -0.0&    2.0&    3.4&   -1.4&    1.9\\
0.09:0.13&  17.900000&    3.4&    1.5&    3.6&    0.8&   -0.7&    1.3&   -0.0&   -0.1&   -0.0&    1.9&    2.9&   -0.5&    1.9\\
0.13:0.18&  13.700000&    3.6&    2.2&    2.5&    1.4&   -0.4&    0.6&    0.0&   -0.1&    0.0&    1.9&    2.6&   -3.2&    1.9\\
0.18:0.26&  11.300000&    3.3&    2.3&    1.0&    1.1&    0.2&   -0.6&    0.1&   -0.1&    0.1&    1.8&    2.7&    1.3&    1.9\\
0.26:0.36&   8.030000&    3.7&    2.2&    3.0&    1.8&   -0.5&   -1.1&    0.5&    0.1&    0.1&    1.8&    2.8&    0.4&    1.9\\
0.36:0.50&   5.090000&    4.2&    1.9&    5.6&    1.1&    0.9&   -2.1&    1.6&    0.3&   -0.2&    1.8&    3.1&    0.9&    1.9\\
0.50:0.70&   2.900000&    6.0&    3.0&    4.1&    0.4&    0.8&   -5.1&    2.5&    0.2&    0.6&    1.7&    3.2&    5.8&    1.9\\
\hline
\end{tabu}
%\end{center}
\caption[Input single-differential \Dstar cross section as function of $y$]
{Input data used for the combination of the \Dstar single-differential cross section as a function of $y$. 
The tables report for each bin the input differential cross section (${\rm d}\sigma/{\rm d}y$) together with its statistical ($\delta_{stat}$), 
uncorrelated ($\delta_{uncor}$) and all correlated (all other $\delta_{...}$)
%, $XXX \neq stat$, $XXX \neq uncor$) 
uncertainties; the theoretical uncertainties from the swimming procedure are shown separately ($\delta_{sw}$).}
\label{tab:comb:dstar:single:inputy}
\end{sidewaystable}


==> content/combination/dstar/input/set_h1zeus_z.tex <==
\begin{sidewaystable}[tbp]
\small
%\begin{center}
\tabcolsep1.2mm
\renewcommand*{\arraystretch}{1.1}
\begin{tabu}{|>{$}c<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|} \hline
\multicolumn{16}{|c|}{H1 HERA-II (datasets I+II)}\\ \hline
z(\Dstar)&{\rm d}\sigma/{\rm d}z(\Dstar)&%\multicolumn{14}{c|}{$\delta$}\\ \cline{3-16}
\delta_{stat}&\delta_{uncor}&\delta_{1}&\delta_{2}&\delta_{3}&\delta_{4}&\delta_{5}&\delta_{6}&\delta_{7}&\delta_{8}&\delta_{9}&\delta_{10}&\delta_{sw}&\delta_{11}\\ \hline
&[$\SI{}{nb}]$&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]\\ \hline
0.000:0.100&   3.479279&   12.5&    5.0&    2.9&    3.2&    1.0&    0.7&    0.8&   -1.4&   -0.0&    4.2&   -0.7&   -3.5&    0.2&    0.7\\
0.100:0.200&   7.307088&    6.2&    5.0&    2.9&    3.2&    1.0&    0.9&    0.9&   -1.8&   -0.0&    0.6&   -0.8&   -4.1&    0.2&    0.5\\
0.200:0.325&   8.506860&    4.4&    5.0&    2.9&    3.2&    1.0&    1.0&    1.1&   -1.9&   -0.0&   -3.7&   -1.0&   -2.5&    0.4&    0.4\\
0.325:0.450&   7.895236&    4.1&    5.0&    2.9&    3.2&    1.0&    1.2&    1.1&   -2.5&   -0.0&   -3.6&   -0.4&   -2.3&    0.4&    0.5\\
0.450:0.575&   7.723692&    3.8&    5.0&    2.9&    3.2&    1.0&    0.3&    1.0&   -1.1&   -0.0&   -3.8&    0.1&   -1.1&    0.2&    0.5\\
0.575:0.800&   4.337003&    3.1&    5.0&    2.9&    3.2&    1.0&   -1.6&    0.8&    2.4&   -0.0&   -4.2&   -0.7&   -1.0&    0.7&    0.8\\
0.800:1.000&   0.928485&   7.4&    5.0&    2.9&    3.2&    1.0&  -13.5&   -0.4&   21.1&   -0.0&    0.2&   -2.7&   -7.2&    2.5&    1.0\\
\hline
\end{tabu}

\begin{tabu}{|>{$}c<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|} \hline
\multicolumn{15}{|c|}{ZEUS HERA-II (datasets III)}\\ \hline
z(\Dstar)&{\rm d}\sigma/{\rm d}z(\Dstar)&%\multicolumn{13}{c|}{$\delta$}\\ \cline{3-15}
\delta_{stat}&\delta_{uncor}&\delta_{12}&\delta_{13}&\delta_{14}&\delta_{15}&\delta_{16}&\delta_{17}&\delta_{18}&\delta_{19}&\delta_{20}&\delta_{21}&\delta_{22}\\ \hline
&[$\SI{}{nb}]$&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]\\ \hline
0.000:0.100&   3.000000&   12.3&    5.9&    5.9&    2.8&   -1.4&   -4.7&    1.8&   -0.0&    0.2&    2.4&    3.4&    2.4&    1.9\\
0.100:0.200&   6.800000&    6.1&    2.3&    9.8&    1.6&   -0.8&   -3.5&    1.2&   -0.4&    0.2&    2.2&    2.9&    1.3&    1.9\\
0.200:0.325&   8.180000&    3.5&    2.3&    4.3&    1.9&   -0.5&   -2.2&    0.9&   -0.2&    0.1&    2.0&    2.9&    0.9&    1.9\\
0.325:0.450&   9.100000&    2.5&    1.5&   -0.3&    1.3&   -0.4&   -0.6&    0.4&    0.1&   -0.1&    1.8&    2.9&    0.8&    1.9\\
0.450:0.575&   9.140000&    1.3&    1.3&    1.1&    0.6&   -0.3&    1.5&    0.1&    0.1&   -0.1&    1.7&    2.9&    1.5&    1.9\\
0.575:0.800&   5.120000&    1.4&    2.1&    1.4&   -1.6&   -0.3&    4.0&    0.2&    0.3&   -0.1&    1.5&    2.9&    2.5&    1.9\\
0.800:1.000&   0.630000&   9.1&    5.7&   -1.0&   -7.0&   -0.2&    5.6&    0.0&    1.1&    0.3&    1.4&    3.1&    2.7&    1.9\\
\hline
\end{tabu}
%\end{center}
\caption[Input single-differential \Dstar cross section as function of $z(\Dstar)$]
{Input data used for the combination of the \Dstar single-differential cross section as a function of $z(\Dstar)$. 
The tables report for each bin the input differential cross section (${\rm d}\sigma/{\rm d}z(\Dstar)$) together with its statistical ($\delta_{stat}$), 
uncorrelated ($\delta_{uncor}$) and all correlated (all other $\delta_{...}$)
%, $XXX \neq stat$, $XXX \neq uncor$) 
uncertainties; the theoretical uncertainties from the swimming procedure are shown separately ($\delta_{sw}$).}
\label{tab:comb:dstar:single:inputz}
\end{sidewaystable}


==> content/combination/dstar/input/set_zeus9800_q2y.tex <==
%\begin{landscape}
\begin{table}[tbp]
%\footnotesize
%\begin{center}
\tabcolsep1.2mm
\renewcommand*{\arraystretch}{1.1}
\begin{tabu}{|>{$}c<{$}|>{$}c<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|} \hline
\multicolumn{11}{|c|}{ZEUS 9800 (dataset IV)}\\ \hline
Q^2&y&\frac{{\rm d}^2\sigma}{{\rm d}Q^2{\rm d}y}&%\multicolumn{8}{c|}{$\delta$}\\ \cline{4-11}
\delta_{stat}&\delta_{uncor}&\delta_{23}&\delta_{24}&\delta_{25}&\delta_{26}&\delta_{27}&\delta_{28}\\ \hline
[$\SI{}{GeV^2}$]&&[$\SI{}{nb/GeV^2}]$&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]\\ \hline
   1.5:   3.5&  0.02:0.09&   0.654477&    7.4&   10.7&    2.2&   -0.0&    0.0&    0.0&    0.0&   -0.0\\
   1.5:   3.5&  0.09:0.16&   0.755615&    6.6&    9.2&    2.2&   -0.2&    0.3&    0.1&    0.2&   -0.2\\
   1.5:   3.5&  0.16:0.32&   0.940910&    8.3&    8.8&    2.2&   -0.3&    0.6&   -0.1&    0.1&    0.1\\
   1.5:   3.5&  0.32:0.70&   0.687336&   11.1&   17.4&    2.2&   -0.1&    0.2&   -0.0&    0.1&   -0.0\\
   3.5:   5.5&  0.02:0.09&   0.305303&    6.8&    9.1&    2.2&    0.8&   -0.7&   -0.2&    0.1&    0.3\\
   3.5:   5.5&  0.09:0.16&   0.271557&    6.5&    4.6&    2.2&   -0.3&   -0.7&    0.2&    0.2&    0.3\\
   3.5:   5.5&  0.16:0.32&   0.342211&    9.0&   18.2&    2.2&   -0.6&    0.4&   -0.3&    0.4&    0.1\\
   3.5:   5.5&  0.32:0.70&   0.258784&   12.1&    8.4&    2.2&   -0.3&   -0.1&    0.1&    0.2&    0.5\\
   5.5:   9.0&  0.32:0.70&   0.296152&   10.3&   16.1&    2.2&    0.5&   -1.6&    0.2&    0.2&    0.7\\
   9.0:  14.0&  0.09:0.16&   0.187517&    7.0&    4.6&    2.2&   -0.3&    0.4&   -0.1&    0.2&   -0.2\\
   9.0:  14.0&  0.16:0.32&   0.312658&    9.6&   14.2&    2.2&   -0.8&    1.4&   -0.1&    0.3&   -0.2\\
   9.0:  14.0&  0.32:0.70&   0.265379&   13.8&   10.9&    2.2&   -0.2&    0.4&   -0.1&    0.2&   -0.2\\
  14.0:  23.0&  0.09:0.16&   0.171290&    6.1&    8.7&    2.2&   -0.2&   -0.1&    0.3&    0.4&    0.3\\
  14.0:  23.0&  0.16:0.32&   0.234964&   11.0&   24.8&    2.2&   -0.6&    0.8&   -0.1&    0.4&   -0.4\\
  14.0:  23.0&  0.32:0.70&   0.177335&   16.9&   23.1&    2.2&   -0.4&    0.6&    0.2&    0.3&   -0.4\\
  23.0:  45.0&  0.05:0.09&   0.097058&    7.1&    8.8&    2.2&    2.4&    0.3&    0.1&    0.6&    0.1\\
  23.0:  45.0&  0.09:0.16&   0.159526&    6.9&    5.1&    2.2&   -0.6&   -0.5&   -0.1&    0.1&   -0.2\\
  23.0:  45.0&  0.16:0.32&   0.265285&    7.8&    8.6&    2.2&   -0.8&    0.7&    0.3&    0.2&   -0.3\\
  23.0:  45.0&  0.32:0.70&   0.252602&   11.5&    9.2&    2.2&   -0.4&    0.7&   -0.0&    0.2&   -0.2\\
  45.0: 100.0&  0.16:0.32&   0.149621&    9.8&   14.8&    2.2&    0.3&    0.1&    0.2&    0.1&    0.1\\
  45.0: 100.0&  0.32:0.70&   0.129460&   14.2&   20.3&    2.2&    0.4&   -0.5&    0.1&    0.1&   -0.1\\
 100.0: 158.0&  0.02:0.32&   0.083083&   11.3&   13.9&    2.2&    0.2&    0.4&    0.1&    0.1&    0.3\\
 100.0: 158.0&  0.32:0.70&   0.032379&   23.3&   22.4&    2.2&    0.5&    0.5&    0.4&    0.1&    0.2\\
 251.0:1000.0&  0.02:0.26&   0.037960&   22.0&   13.0&    2.2&    0.7&   -0.2&   -0.2&    0.6&    0.2\\
 251.0:1000.0&  0.26:0.70&   0.052195&   18.4&   18.6&    2.2&    0.3&   -0.3&   -0.1&    0.3&    0.1\\
\hline
\end{tabu}
%\end{center}
\caption[Input ZEUS 98--00 double-differential \Dstar cross section]
{Input data ZEUS 98--00 (dataset IV) used for the combination of the \Dstar double-differential cross section as a function of $Q^2$ and $y$. 
The table reports for each bin the input differential cross section ($\frac{{\rm d}^2\sigma}{{\rm d}Q^2{\rm d}y}$) together with its statistical ($\delta_{stat}$), 
uncorrelated ($\delta_{uncor}$) and all correlated (all other $\delta_{...}$)
%, $XXX \neq stat$, $XXX \neq uncor$) 
uncertainties.}
\label{tab:comb:dstar:single:inputq2yzeus9800}
\end{table}
%\end{landscape}


==> content/combination/dstar/input/set_zeushera2_q2y.tex <==
\begin{sidewaystable}[tbp]
\footnotesize
%\begin{center}
\tabcolsep1.2mm
\renewcommand*{\arraystretch}{0.96}
\begin{tabu}{|>{$}c<{$}|>{$}c<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|} \hline
\multicolumn{21}{|c|}{ZEUS HERA-II (dataset III)}\\ \hline
Q^2&y&\frac{{\rm d}^2\sigma}{{\rm d}Q^2{\rm d}y}&%\multicolumn{18}{c|}{$\delta$}\\ \cline{4-21}
\delta_{stat}&\delta_{uncor}&\delta_{12}&\delta_{13}&\delta_{14}&\delta_{15}&\delta_{16}&\delta_{17}&\delta_{18}&\delta_{19}&\delta_{20}&\delta_{21}&\delta_{22}&\delta_{24}&\delta_{25}&\delta_{26}&\delta_{27}&\delta_{28}\\ \hline
[$\SI{}{GeV^2}$]&&[$\SI{}{nb/GeV^2}]$&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]\\ \hline
   5.5:   9.0&  0.02:0.05&   0.099573&   23.0&   16.6&    2.0&   -4.2&    1.8&   12.3&    0.0&    0.1&    0.0&    2.5&    2.5&    2.2&    1.9&    0.0&   -0.2&    0.1&    0.1&   -0.2\\
   5.5:   9.0&  0.05:0.09&   0.231647&   10.0&    8.8&    2.0&   -2.3&    5.1&    4.0&    0.0&   -0.8&   -0.1&    2.4&    2.1&   -1.6&    1.9&    0.3&    0.1&   -0.1&    0.1&   -0.2\\
   5.5:   9.0&  0.09:0.16&   0.349456&    6.0&    4.2&    2.0&    0.8&    4.0&    3.4&    0.0&   -1.5&    0.1&    2.3&    1.8&   -2.0&    1.9&   -0.0&    0.4&   -0.1&    0.1&   -0.2\\
   5.5:   9.0&  0.16:0.32&   0.457092&    5.3&    4.1&    2.0&    0.9&    2.9&    0.9&    0.5&   -1.8&    0.0&    2.2&    1.8&    0.7&    1.9&    0.1&    0.1&    0.0&    0.1&   -0.2\\
   5.5:   9.0&  0.32:0.70&   0.378328&    6.8&    3.1&    2.0&    0.4&    1.9&    1.7&    2.4&   -1.5&    0.0&    2.0&    1.9&    3.1&    1.9&    0.3&    0.1&    0.1&    0.1&   -0.2\\
   9.0:  14.0&  0.02:0.05&   0.108000&   14.0&    7.9&    2.0&   -4.7&   -7.3&   11.0&    0.0&   -0.7&    0.1&    2.2&    2.4&    1.4&    1.9&   -0.0&   -0.0&   -0.0&    0.0&   -0.0\\
   9.0:  14.0&  0.05:0.09&   0.178000&    6.5&    4.3&    2.0&   -1.5&   -1.9&    3.2&    0.0&   -1.2&    0.0&    2.2&    2.0&   -1.6&    1.9&   -0.0&   -0.0&   -0.0&    0.0&   -0.0\\
   9.0:  14.0&  0.09:0.16&   0.220000&    5.8&    2.8&    2.0&   -0.1&   -0.3&   -0.6&    0.0&   -1.7&   -0.2&    2.1&    1.7&   -2.0&    1.9&   -0.0&   -0.0&   -0.0&    0.0&   -0.0\\
   9.0:  14.0&  0.16:0.32&   0.352000&    5.1&    2.1&    2.0&    0.7&   -0.5&   -0.5&    0.1&   -1.9&   -0.1&    2.1&    1.8&    0.4&    1.9&   -0.0&   -0.0&   -0.0&    0.0&   -0.0\\
   9.0:  14.0&  0.32:0.70&   0.307000&    7.2&    2.0&    2.0&   -0.5&    1.1&   -3.8&    1.6&   -2.0&    0.3&    1.9&    1.8&    2.8&    1.9&   -0.0&   -0.0&   -0.0&    0.0&   -0.0\\
  14.0:  23.0&  0.02:0.05&   0.065100&   15.0&    7.7&    2.0&   -2.7&   -6.4&   11.5&    0.0&   -0.8&    0.2&    2.1&    2.4&    1.7&    1.9&   -0.0&   -0.0&   -0.0&    0.0&   -0.0\\
  14.0:  23.0&  0.05:0.09&   0.160000&    6.4&    3.5&    2.0&   -1.1&   -3.8&    3.9&    0.0&   -1.9&    0.1&    2.1&    2.0&   -1.7&    1.9&   -0.0&   -0.0&   -0.0&    0.0&   -0.0\\
  14.0:  23.0&  0.09:0.16&   0.205000&    5.6&    2.6&    2.0&    0.4&   -0.8&    1.3&    0.0&   -2.3&   -0.1&    2.0&    1.7&   -2.0&    1.9&   -0.0&   -0.0&   -0.0&    0.0&   -0.0\\
  14.0:  23.0&  0.16:0.32&   0.267000&    5.9&    2.5&    2.0&    1.3&   -0.6&   -0.9&    0.3&   -2.6&    0.2&    1.9&    1.7&    0.4&    1.9&   -0.0&   -0.0&   -0.0&    0.0&   -0.0\\
  14.0:  23.0&  0.32:0.70&   0.249999&    7.4&    3.9&    2.0&    0.4&    1.7&   -2.9&    1.9&   -2.7&    0.2&    1.9&    1.8&    2.9&    1.9&   -0.0&   -0.0&   -0.0&    0.0&   -0.0\\
  23.0:  45.0&  0.02:0.05&   0.037100&   29.0&   15.0&    2.0&   -0.4&  -11.5&    9.5&    0.0&   -0.6&   -0.3&    1.9&    2.2&    1.7&    1.9&   -0.0&   -0.0&   -0.0&    0.0&   -0.0\\
  23.0:  45.0&  0.05:0.09&   0.134000&    7.0&    2.3&    2.0&   -2.4&   -4.8&    4.6&    0.0&   -1.6&   -0.3&    1.8&    1.9&   -1.4&    1.9&   -0.0&   -0.0&   -0.0&    0.0&   -0.0\\
  23.0:  45.0&  0.09:0.16&   0.196000&    5.3&    1.5&    2.0&   -0.3&   -1.8&    1.1&    0.0&   -1.7&    0.3&    1.8&    1.6&   -2.1&    1.9&   -0.0&   -0.0&   -0.0&    0.0&   -0.0\\
  23.0:  45.0&  0.16:0.32&   0.275000&    5.1&    1.5&    2.0&    0.1&    0.4&   -1.2&    0.2&   -1.8&    0.2&    1.8&    1.8&    0.4&    1.9&   -0.0&   -0.0&   -0.0&    0.0&   -0.0\\
  23.0:  45.0&  0.32:0.70&   0.283998&    6.1&    2.8&    2.0&    0.2&   -1.1&   -3.5&    1.3&   -1.7&   -0.2&    1.8&    1.8&    2.4&    1.9&   -0.0&   -0.0&   -0.0&    0.0&   -0.0\\
  45.0: 100.0&  0.02:0.05&   0.014200&   38.0&   13.9&    2.0&   -3.4&   18.2&   26.2&    0.0&   -2.2&    0.0&    1.5&    2.0&    3.5&    1.9&   -0.0&   -0.0&   -0.0&    0.0&   -0.0\\
  45.0: 100.0&  0.05:0.09&   0.072101&   11.6&    5.0&    2.0&   -0.2&   -4.0&    4.2&    0.0&   -1.4&    0.1&    1.5&    1.8&   -1.6&    1.9&   -0.0&   -0.0&   -0.0&    0.0&   -0.0\\
  45.0: 100.0&  0.09:0.16&   0.086998&    8.4&    2.4&    2.0&    0.0&   -2.4&    1.1&    0.0&   -1.9&    0.3&    1.5&    1.5&   -2.1&    1.9&   -0.0&   -0.0&   -0.0&    0.0&   -0.0\\
  45.0: 100.0&  0.16:0.32&   0.182002&    5.7&    3.4&    2.0&    0.0&   -1.9&   -0.7&    0.0&   -2.3&    0.7&    1.6&    1.5&    0.2&    1.9&   -0.0&   -0.0&   -0.0&    0.0&   -0.0\\
  45.0: 100.0&  0.32:0.70&   0.174996&    7.6&    3.8&    2.0&    0.7&   -0.8&   -3.2&    0.9&   -2.7&    0.7&    1.7&    1.6&    2.9&    1.9&   -0.0&   -0.0&   -0.0&    0.0&   -0.0\\
 100.0: 158.0&  0.02:0.32&   0.074570&   11.0&    5.2&    2.0&   -0.2&   -4.4&    1.7&   -0.2&   -1.3&    0.0&    1.3&    1.4&   -0.2&    1.9&   -0.2&   -0.2&    0.0&    0.0&   -0.0\\
 100.0: 158.0&  0.32:0.70&   0.051533&   16.0&    5.6&    2.0&    0.4&   -2.5&   -5.3&    1.1&   -1.3&    3.2&    1.4&    1.5&    2.9&    1.9&   -0.1&   -0.1&   -0.1&    0.0&   -0.1\\
 158.0: 251.0&  0.02:0.30&   0.049788&   14.0&    3.8&    2.0&    0.6&   -4.3&    0.8&    0.1&   -0.9&    1.0&    1.2&    1.3&    0.1&    1.9&   -0.0&   -0.0&   -0.0&    0.0&   -0.0\\
 158.0: 251.0&  0.30:0.70&   0.037312&   17.0&    4.0&    2.0&    0.5&    0.6&   -2.6&    1.0&   -1.0&    0.7&    1.4&    1.4&    3.0&    1.9&   -0.0&   -0.0&   -0.0&    0.0&   -0.0\\
 251.0:1000.0&  0.02:0.26&   0.026341&   24.0&    7.3&    2.0&   -1.0&   -5.9&    2.2&    0.0&    0.1&    1.3&    1.2&    1.3&   -0.3&    1.9&   -0.3&   -0.3&   -0.1&    0.1&    0.1\\
 251.0:1000.0&  0.26:0.70&   0.049167&   21.0&    5.8&    2.0&   -0.5&   -3.8&   -4.3&    1.4&   -1.0&    0.1&    1.4&    1.4&    0.9&    1.9&   -0.1&   -0.1&    0.1&    0.1&   -0.1\\
\hline
\end{tabu}
%\end{center}
\caption[Input ZEUS HERA-II double-differential \Dstar cross section]
{Input data ZEUS HERA-II (dataset III) used for the combination of the \Dstar double-differential cross section as a function of $Q^2$ and $y$. 
The table reports for each bin the input differential cross section ($\frac{{\rm d}^2\sigma}{{\rm d}Q^2{\rm d}y}$) together with its statistical ($\delta_{stat}$), 
uncorrelated ($\delta_{unc}$) and all correlated (all other $\delta_{...}$)
%, $XXX \neq stat$, $XXX \neq uncor$) 
uncertainties.}
\label{tab:comb:dstar:single:inputq2yzeushera2}
\end{sidewaystable}


==> content/combination/dstar/tabs/highq2corr.tex <==
\begin{table}[tbp]
\footnotesize
%\begin{center}
\tabcolsep0.87mm
\renewcommand*{\arraystretch}{0.98}
%\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|} \hline
%\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|>{$}r<{$}|} \hline
\begin{tabular}{|>{$}c<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|} \hline
\multicolumn{16}{|c|}{${\rm d}\sigma/{\rm d}p_T(\Dstar)$}\\ \hline
p_T(\Dstar)&C&\delta_{mc}^{+}&\delta_{mc}^{-}&\delta_{mu}^{+}&\delta_{mu}^{-}&\delta_{as}^{+}&\delta_{as}^{-}&\delta_{ak}^{+}&\delta_{ak}^{-}&\delta_{bn}^{+}&\delta_{bn}^{-}&\delta_{kt}^{+}&\delta_{kt}^{-}&\delta_{tot}^{+}&\delta_{tot}^{-}\\ \hline
[$\SI{}{GeV}]$&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]\\ \hline
 1.50: 1.88&    1.0&   -2.0&    2.9&   -2.1&    4.6&    0.3&    0.4&   -4.2&    5.5&   -1.5&    3.7&   -0.6&    0.1&    8.6&   -5.3\\
 1.88: 2.28&    1.2&   -2.0&    1.2&   -2.8&    5.0&    0.1&   -0.5&   -4.2&    5.5&   -1.8&    3.9&   -0.3&    0.2&    8.5&   -5.7\\
 2.28: 2.68&    1.3&    0.3&   -0.1&   -2.8&    5.9&    0.2&   -0.5&   -4.1&    5.1&   -2.8&    5.0&    0.1&    0.3&    9.3&   -5.8\\
 2.68: 3.08&    1.9&    0.8&   -0.6&   -3.2&    6.9&    0.6&    0.1&   -3.7&    5.3&   -2.7&    5.3&    0.9&    0.2&   10.3&   -5.6\\
 3.08: 3.50&    2.3&    1.1&   -1.6&   -3.2&    6.2&   -0.2&    0.0&   -4.2&    4.8&   -3.3&    5.9&   -0.1&   -0.7&    9.9&   -6.5\\
 3.50: 4.00&    3.2&    1.0&   -0.9&   -2.6&    5.0&    0.4&    0.0&   -3.9&    5.1&   -3.4&    6.1&    0.1&    0.2&    9.4&   -5.9\\
 4.00: 4.75&    4.5&    1.0&   -1.9&   -2.4&    3.2&    0.1&   -0.3&   -3.7&    3.3&   -3.2&    5.0&   -0.3&   -0.2&    6.9&   -5.8\\
 4.75: 6.00&    9.1&    0.7&   -0.4&    0.1&    1.1&   -0.0&    0.1&   -1.8&    2.1&   -2.2&    2.5&   -0.3&    0.1&    3.5&   -3.1\\
 6.00: 8.00&   21.8&   -0.3&    0.4&    2.1&   -3.5&   -0.1&    0.1&    1.5&   -2.3&    0.9&   -3.3&   -0.1&    0.1&    2.8&   -5.3\\
 8.00:11.00&   37.8&   -1.0&    0.8&    2.6&   -5.3&   -0.2&   -0.0&    5.0&   -6.0&    4.7&   -7.2&    0.2&   -0.2&    7.4&  -10.8\\
11.00:20.00&   54.0&    0.4&    0.1&    1.7&   -5.0&   -0.2&    0.3&    7.3&   -7.5&    4.7&   -4.6&    0.7&   -0.1&    8.8&  -10.1\\
\hline
\hline
\multicolumn{16}{|c|}{${\rm d}\sigma/{\rm d}\eta(\Dstar)$}\\ \hline
\eta(\Dstar)&C&\delta_{mc}^{+}&\delta_{mc}^{-}&\delta_{mu}^{+}&\delta_{mu}^{-}&\delta_{as}^{+}&\delta_{as}^{-}&\delta_{ak}^{+}&\delta_{ak}^{-}&\delta_{bn}^{+}&\delta_{bn}^{-}&\delta_{kt}^{+}&\delta_{kt}^{-}&\delta_{tot}^{+}&\delta_{tot}^{-}\\ \hline
$\SI{}{}$&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]\\ \hline
-1.50:-1.25&    2.5&   -0.8&    1.0&    5.8&   -7.3&   -0.7&    0.2&    0.2&   -0.5&   -0.0&   -0.2&   -0.8&    0.6&    5.9&   -7.4\\
-1.25:-1.00&    3.4&   -0.4&    0.3&    4.6&   -4.9&   -0.1&    0.5&    0.0&   -0.1&   -0.1&   -0.1&   -0.7&    0.1&    4.7&   -4.9\\
-1.00:-0.75&    3.8&   -0.2&    0.5&    3.8&   -3.8&    0.1&    0.7&    0.0&    0.2&   -0.1&    0.0&   -0.0&    0.4&    3.9&   -3.9\\
-0.75:-0.50&    4.2&   -0.2&    0.3&    2.7&   -3.0&   -0.1&    0.1&    0.0&   -0.2&   -0.2&   -0.1&   -0.2&   -0.0&    2.8&   -3.0\\
-0.50:-0.25&    4.9&   -0.2&    0.2&    1.8&   -1.9&   -0.2&    0.1&   -0.0&    0.1&   -0.0&   -0.3&   -0.2&    0.2&    1.8&   -1.9\\
-0.25: 0.00&    5.1&   -0.3&    0.1&    0.9&   -1.2&   -0.1&   -0.1&    0.0&   -0.2&   -0.0&   -0.2&   -0.2&    0.0&    0.9&   -1.3\\
 0.00: 0.25&    5.1&   -0.2&    0.1&    0.2&   -0.2&    0.1&    0.1&   -0.1&    0.1&    0.1&   -0.2&    0.0&    0.1&    0.3&   -0.4\\
 0.25: 0.50&    5.2&    0.1&    0.1&   -0.8&    1.1&    0.0&    0.1&   -0.0&   -0.0&    0.1&    0.0&    0.2&    0.1&    1.1&   -0.8\\
 0.50: 0.75&    4.9&    0.2&    0.0&   -1.5&    1.8&    0.2&   -0.2&    0.1&    0.1&    0.1&   -0.0&    0.2&    0.1&    1.8&   -1.5\\
 0.75: 1.00&    4.8&    0.1&   -0.5&   -2.7&    2.8&    0.1&   -0.1&    0.1&    0.2&    0.1&    0.2&    0.1&   -0.3&    2.8&   -2.8\\
 1.00: 1.25&    3.9&    0.4&   -0.6&   -3.3&    3.4&    0.1&   -0.3&   -0.3&   -0.1&   -0.1&    0.3&    0.1&   -0.4&    3.4&   -3.4\\
 1.25: 1.50&    4.3&    0.7&   -0.6&   -4.5&    5.0&    0.2&   -0.5&    0.1&    0.2&   -0.0&    0.3&    0.8&   -0.3&    5.2&   -4.6\\
\hline
\hline
\multicolumn{16}{|c|}{${\rm d}\sigma/{\rm d}z(\Dstar)$}\\ \hline
z(\Dstar)&C&\delta_{mc}^{+}&\delta_{mc}^{-}&\delta_{mu}^{+}&\delta_{mu}^{-}&\delta_{as}^{+}&\delta_{as}^{-}&\delta_{ak}^{+}&\delta_{ak}^{-}&\delta_{bn}^{+}&\delta_{bn}^{-}&\delta_{kt}^{+}&\delta_{kt}^{-}&\delta_{tot}^{+}&\delta_{tot}^{-}\\ \hline
$\SI{}{}$&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]\\ \hline
0.000:0.100&    5.2&   -2.9&    2.5&   -1.0&    2.7&    0.4&   -0.1&   -1.0&    1.6&    1.0&    0.1&    1.2&   -0.7&    4.4&   -3.3\\
0.100:0.200&    3.7&    1.8&   -1.6&   -2.7&    5.3&    0.4&   -0.3&   -2.5&    3.4&   -1.2&    1.7&    0.2&   -0.1&    6.7&   -4.2\\
0.200:0.325&    3.1&    2.0&   -2.0&   -4.6&    8.2&    0.3&   -0.3&   -4.2&    5.2&   -3.3&    5.8&   -0.1&    0.0&   11.5&   -7.3\\
0.325:0.450&    3.6&    1.9&   -1.9&   -3.9&    6.5&    0.1&   -0.3&   -4.3&    4.7&   -4.2&    7.0&   -0.1&    0.1&   10.8&   -7.4\\
0.450:0.575&    4.0&    1.0&   -1.1&   -1.2&    1.7&   -0.0&    0.1&   -1.9&    1.5&   -2.6&    3.8&   -0.2&    0.1&    4.6&   -3.6\\
0.575:0.800&    6.1&   -1.4&    1.3&    4.1&   -7.4&   -0.3&    0.2&    4.6&   -5.7&    2.9&   -6.3&   -0.2&    0.1&    6.9&  -11.4\\
0.800:1.000&    7.0&   -6.9&    7.3&   14.2&  -24.3&   -1.3&    1.2&   13.5&  -13.6&   15.2&  -19.6&   -0.1&    0.1&   25.9&  -34.8\\
\hline
\hline
\multicolumn{16}{|c|}{${\rm d}\sigma/{\rm d}y$}\\ \hline
y&C&\delta_{mc}^{+}&\delta_{mc}^{-}&\delta_{mu}^{+}&\delta_{mu}^{-}&\delta_{as}^{+}&\delta_{as}^{-}&\delta_{ak}^{+}&\delta_{ak}^{-}&\delta_{bn}^{+}&\delta_{bn}^{-}&\delta_{kt}^{+}&\delta_{kt}^{-}&\delta_{tot}^{+}&\delta_{tot}^{-}\\ \hline
$\SI{}{}$&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]&[\%]\\ \hline
0.02:0.05&    0.5&  -12.2&   11.7&   -4.8&    2.5&    0.5&   -0.6&    2.6&   -3.5&    2.3&   -4.9&    0.3&   -0.1&   12.4&  -14.4\\
0.05:0.09&    2.6&   -4.4&    4.0&   -3.7&    2.3&   -0.2&   -0.3&    0.3&   -0.4&   -0.0&   -0.5&   -0.4&    0.2&    4.7&   -5.8\\
0.09:0.13&    3.4&   -1.7&    1.6&   -2.4&    1.7&   -0.1&   -0.2&   -0.1&    0.1&   -0.2&    0.1&   -0.2&    0.1&    2.4&   -2.9\\
0.13:0.18&    4.0&   -0.6&    0.6&   -1.2&    0.9&    0.0&    0.0&   -0.1&    0.1&   -0.2&    0.0&   -0.1&    0.1&    1.1&   -1.4\\
0.18:0.26&    4.2&    0.1&   -0.1&   -0.1&    0.1&   -0.0&    0.0&   -0.1&    0.1&   -0.0&    0.0&   -0.1&    0.0&    0.2&   -0.2\\
0.26:0.36&    5.4&    0.7&   -0.6&    0.8&   -0.6&    0.0&    0.1&   -0.1&    0.1&    0.0&    0.1&    0.0&   -0.0&    1.1&   -0.9\\
0.36:0.50&    6.6&    1.1&   -1.1&    1.6&   -1.2&   -0.0&    0.1&   -0.0&    0.1&    0.0&    0.1&    0.1&   -0.0&    2.0&   -1.7\\
0.50:0.70&    8.1&    1.9&   -1.8&    1.7&   -0.9&    0.1&    0.0&    0.0&   -0.0&    0.1&    0.1&    0.3&   -0.2&    2.5&   -2.0\\
\hline
\end{tabular}
%\end{center}
\caption[Contributions from high-$Q^2$ region and their uncertainties for high-$Q^2$ swimming]
{Contributions from the high-$Q^2$ region ($C$) and their uncertainties for high-$Q^2$ swimming for H1 HERA-II measurement 
(see Section~\ref{sec:comb:dstar:single:det} for more details).}
\label{tab:comb:dstar:single:highq2}
\end{table}


==> content/combination/dstar/tabs/swimming/swimming_zeus9697_reduced.tex <==
\begin{table}[tbp]
\begin{center}
\tabcolsep1.1mm
\renewcommand*{\arraystretch}{1.2}
%\begin{tabular}{|l|l|l|l|l|l|l|l|l|} \hline
\begin{tabular}{|l|l|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|} \hline
\multicolumn{9}{c}{ZEUS 9697 (dataset V)} \\ \hline
%Input bin & Output bin & $P$ [\%]    & $E$ [\%] & $F_{\rm sw}$ & $\delta^{+} F_{\rm sw}$ & $\delta^{-} F_{\rm sw}$ [\%] & $\delta_{uncor}$ [\%] &  $\delta F_{\rm sw}/\delta_{uncor}$  [\%] \\ \hline
Input bin & Output bin & P~[\%]    & E~[\%] & F_{\rm sw} & \delta^{+} F_{\rm sw} & \delta^{-} F_{\rm sw}~[\%] & \delta_{uncor}~[\%] &  \delta F_{\rm sw}/\delta_{uncor}~[\%] \\ \hline
          1 &     1 &   54.4 &   95.8 &   0.910 &   0.7 &  -2.6 &  21.9 &  11.9 \\ \hline
          2 &     3 &   36.4 &   57.4 &   0.642 &   1.5 &  -1.6 &  26.2 &   6.2 \\ \hline
          3 &     4 &   44.1 &   96.2 &   0.694 &   0.9 &  -1.1 &  21.5 &   5.1 \\ \hline
          4 &     5 &   59.2 &   96.0 &   1.195 &   0.5 &  -1.8 &  22.6 &   7.9 \\ \hline
          5 &     6 &   38.2 &   64.9 &   1.392 &   0.9 &  -0.7 &  22.4 &   4.0 \\ \hline
          6 &     8 &   43.5 &   95.9 &   0.862 &   1.9 &  -1.5 &  18.5 &  10.1 \\ \hline
          7 &    11 &   39.7 &   54.7 &   0.963 &   5.0 &  -3.7 &  22.4 &  22.2 \\ \hline
          8 &    12 &   54.9 &   62.2 &   2.157 &   1.6 &  -3.4 &  20.5 &  16.7 \\ \hline
          9 &    15 &   46.5 &   95.6 &   1.098 &   2.9 &  -3.0 &  17.8 &  16.9 \\ \hline
         10 &    17 &   51.4 &   51.6 &   0.753 &   2.2 &  -1.7 &  24.9 &   8.9 \\ \hline
         11 &    18 &   61.0 &   95.6 &   0.794 &   1.7 &  -2.2 &  18.0 &  12.2 \\ \hline
         12 &    20 &   47.6 &   88.5 &   1.083 &   2.6 &  -3.0 &  23.6 &  12.8 \\ \hline
         13 &    21 &   48.2 &   59.9 &   1.218 &   1.5 &  -0.2 &  28.8 &   5.2 \\ \hline
         14 &    23 &   61.3 &   87.9 &   0.767 &   3.0 &  -1.3 &  34.9 &   8.5 \\ \hline
         15 &    25 &   45.7 &   92.6 &   1.110 &   2.6 &  -2.1 &  20.9 &  12.6 \\ \hline
         16 &    27 &   48.2 &   47.8 &   0.756 &   1.4 &  -1.1 &  18.3 &   7.4 \\ \hline
         17 &    28 &   57.8 &   92.7 &   0.772 &   2.2 &  -0.8 &  18.2 &  12.2 \\ \hline
         18 &    31 &   35.7 &   87.1 &   1.033 &   1.5 &  -2.1 &  17.4 &  12.2 \\ \hline
         19 &    33 &   63.0 &   85.8 &   0.761 &   1.0 &  -0.8 &  28.0 &   3.6 \\ \hline
         20 &    34 &   61.4 &   68.8 &   1.182 &   2.0 &  -0.3 &  23.1 &   8.7 \\ \hline
         21 &    35 &   42.2 &   94.2 &   1.056 &   0.0 &  -1.3 &  28.4 &   4.5 \\ \hline
\hline         
\multicolumn{9}{c}{H1 HERA-I (dataset VI)} \\ \hline
%Input bin & Output bin & $P$ [\%]    & $E$ [\%] & $F_{\rm sw}$ & $\delta^{+} F_{\rm sw}$ & $\delta^{-} F_{\rm sw}$ [\%] & $\delta_{uncor}$ [\%] &  $\delta F_{\rm sw}/\delta_{uncor}$  [\%] \\ \hline
Input bin & Output bin & P~[\%]    & E~[\%] & F_{\rm sw} & \delta^{+} F_{\rm sw} & \delta^{-} F_{\rm sw}~[\%] & \delta_{uncor}~[\%] &  \delta F_{\rm sw}/\delta_{uncor}~[\%] \\ \hline
      4,  5 &     2 &   37.6 &   58.9 &   1.338 &   1.2 &  -0.9 &  13.1 &   8.8 \\ \hline
          3 &     3 &   67.4 &   38.1 &   1.385 &   1.3 &  -0.4 &  10.8 &  11.9 \\ \hline
      1,  2 &     4 &   62.1 &   64.6 &   1.101 &   1.0 &  -1.1 &  26.4 &   4.1 \\ \hline
          9 &    11 &   39.1 &   71.2 &   0.898 &   1.0 &  -1.1 &  12.1 &   9.0 \\ \hline
          8 &    12 &   44.4 &   76.8 &   0.833 &   1.6 &  -1.2 &  12.5 &  12.6 \\ \hline
      6,  7 &    13 &   40.5 &   91.9 &   0.667 &   2.0 &  -1.4 &  15.9 &  12.9 \\ \hline
         12 &    15 &   33.9 &   74.6 &   1.551 &   1.3 &  -1.8 &  15.2 &  12.1 \\ \hline
         10 &    18 &   31.5 &   42.1 &   0.845 &   2.8 &  -2.6 &  12.5 &  22.1 \\ \hline
     11, 14 &    22 &   36.7 &   80.3 &   1.396 &   0.4 &  -0.7 &  11.7 &   6.3 \\ \hline
         13 &    23 &   68.6 &   31.7 &   1.865 &   1.4 &  -1.5 &  24.8 &   6.2 \\ \hline
         15 &    27 &   21.3 &   39.0 &   0.416 &   2.5 &  -2.5 &  13.8 &  18.4 \\ \hline
         17 &    31 &   27.2 &   99.5 &   0.929 &   1.0 &  -1.1 &  15.5 &   6.9 \\ \hline
         16 &    33 &   36.7 &   81.7 &   0.484 &   2.3 &  -2.0 &  21.5 &  10.7 \\ \hline
\end{tabular}
\end{center}
\caption[\chisq, \ndof and the corresponding $\chi^2$-probabilities for the combinations of the single-differential \Dstar cross sections]
{Purity ($P$), efficiency ($E$), swimming factors ($F_{\rm sw}$), swimming uncertainties ($\delta^{+} F_{\rm sw}$, $\delta^{-} F_{\rm sw}$), 
uncorrelated experimental uncertainties ($\delta_{uncor}$) and the ratio of the swimming uncertainty to the experimental uncorrelated one ($\delta F_{\rm sw}/\delta_{uncor}$) 
for the \Dstar double-differential cross sections for datasets V and VI. The bin numbering scheme is consistent with Figs.~\ref{fig:comb:dstar:double:swimzd97_1} to~\ref{fig:comb:dstar:double:swimzd97_1}.}
\label{tab:comb:dstar:double:swimzd97}
\end{table}


==> content/combination/dstar/tabs/swimming/swimming_zeus9697h1hera1_reduced.tex <==
\begin{table}[tbp]
%\small
\begin{center}
\tabcolsep1.1mm
\renewcommand*{\arraystretch}{0.99}
%\begin{tabular}{|l|l|l|l|l|l|l|l|l|} \hline
\begin{tabular}{|l|l|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|} \hline
\multicolumn{9}{|c|}{ZEUS 9697 (dataset V)} \\ \hline
%Input bin & Output bin & $P$ [\%]    & $E$ [\%] & $F_{\rm sw}$ & $\delta^{+} F_{\rm sw}$ & $\delta^{-} F_{\rm sw}$ [\%] & $\delta_{uncor}$ [\%] &  $\delta F_{\rm sw}/\delta_{uncor}$  [\%] \\ \hline
Input bin & Output bin & P~[\%]    & E~[\%] & F_{\rm sw} & \delta^{+} F_{\rm sw} & \delta^{-} F_{\rm sw}~[\%] & \delta_{uncor}~[\%] &  \delta F_{\rm sw}/\delta_{uncor}~[\%] \\ \hline
          1 &     1 &   54.4 &   95.8 &   0.910 &   0.7 &  -2.6 &  21.9 &  11.9 \\ \hline
          2 &     3 &   36.4 &   57.4 &   0.642 &   1.5 &  -1.6 &  26.2 &   6.2 \\ \hline
          3 &     4 &   44.1 &   96.2 &   0.694 &   0.9 &  -1.1 &  21.5 &   5.1 \\ \hline
          4 &     5 &   59.2 &   96.0 &   1.195 &   0.5 &  -1.8 &  22.6 &   7.9 \\ \hline
          5 &     6 &   38.2 &   64.9 &   1.392 &   0.9 &  -0.7 &  22.4 &   4.0 \\ \hline
          6 &     8 &   43.5 &   95.9 &   0.862 &   1.9 &  -1.5 &  18.5 &  10.1 \\ \hline
          7 &    11 &   39.7 &   54.7 &   0.963 &   5.0 &  -3.7 &  22.4 &  22.2 \\ \hline
          8 &    12 &   54.9 &   62.2 &   2.157 &   1.6 &  -3.4 &  20.5 &  16.7 \\ \hline
          9 &    15 &   46.5 &   95.6 &   1.098 &   2.9 &  -3.0 &  17.8 &  16.9 \\ \hline
         10 &    17 &   51.4 &   51.6 &   0.753 &   2.2 &  -1.7 &  24.9 &   8.9 \\ \hline
         11 &    18 &   61.0 &   95.6 &   0.794 &   1.7 &  -2.2 &  18.0 &  12.2 \\ \hline
         12 &    20 &   47.6 &   88.5 &   1.083 &   2.6 &  -3.0 &  23.6 &  12.8 \\ \hline
         13 &    21 &   48.2 &   59.9 &   1.218 &   1.5 &  -0.2 &  28.8 &   5.2 \\ \hline
         14 &    23 &   61.3 &   87.9 &   0.767 &   3.0 &  -1.3 &  34.9 &   8.5 \\ \hline
         15 &    25 &   45.7 &   92.6 &   1.110 &   2.6 &  -2.1 &  20.9 &  12.6 \\ \hline
         16 &    27 &   48.2 &   47.8 &   0.756 &   1.4 &  -1.1 &  18.3 &   7.4 \\ \hline
         17 &    28 &   57.8 &   92.7 &   0.772 &   2.2 &  -0.8 &  18.2 &  12.2 \\ \hline
         18 &    31 &   35.7 &   87.1 &   1.033 &   1.5 &  -2.1 &  17.4 &  12.2 \\ \hline
         19 &    33 &   63.0 &   85.8 &   0.761 &   1.0 &  -0.8 &  28.0 &   3.6 \\ \hline
         20 &    34 &   61.4 &   68.8 &   1.182 &   2.0 &  -0.3 &  23.1 &   8.7 \\ \hline
         21 &    35 &   42.2 &   94.2 &   1.056 &   0.0 &  -1.3 &  28.4 &   4.5 \\ \hline
\hline         
\multicolumn{9}{|c|}{H1 HERA-I (dataset VI)} \\ \hline
%Input bin & Output bin & $P$ [\%]    & $E$ [\%] & $F_{\rm sw}$ & $\delta^{+} F_{\rm sw}$ & $\delta^{-} F_{\rm sw}$ [\%] & $\delta_{uncor}$ [\%] &  $\delta F_{\rm sw}/\delta_{uncor}$  [\%] \\ \hline
Input bin & Output bin & P~[\%]    & E~[\%] & F_{\rm sw} & \delta^{+} F_{\rm sw} & \delta^{-} F_{\rm sw}~[\%] & \delta_{uncor}~[\%] &  \delta F_{\rm sw}/\delta_{uncor}~[\%] \\ \hline
      4,  5 &     2 &   37.6 &   58.9 &   1.338 &   1.2 &  -0.9 &  13.1 &   8.8 \\ \hline
          3 &     3 &   67.4 &   38.1 &   1.385 &   1.3 &  -0.4 &  10.8 &  11.9 \\ \hline
      1,  2 &     4 &   62.1 &   64.6 &   1.101 &   1.0 &  -1.1 &  26.4 &   4.1 \\ \hline
          9 &    11 &   39.1 &   71.2 &   0.898 &   1.0 &  -1.1 &  12.1 &   9.0 \\ \hline
          8 &    12 &   44.4 &   76.8 &   0.833 &   1.6 &  -1.2 &  12.5 &  12.6 \\ \hline
      6,  7 &    13 &   40.5 &   91.9 &   0.667 &   2.0 &  -1.4 &  15.9 &  12.9 \\ \hline
         12 &    15 &   33.9 &   74.6 &   1.551 &   1.3 &  -1.8 &  15.2 &  12.1 \\ \hline
         10 &    18 &   31.5 &   42.1 &   0.845 &   2.8 &  -2.6 &  12.5 &  22.1 \\ \hline
     11, 14 &    22 &   36.7 &   80.3 &   1.396 &   0.4 &  -0.7 &  11.7 &   6.3 \\ \hline
         13 &    23 &   68.6 &   31.7 &   1.865 &   1.4 &  -1.5 &  24.8 &   6.2 \\ \hline
         15 &    27 &   21.3 &   39.0 &   0.416 &   2.5 &  -2.5 &  13.8 &  18.4 \\ \hline
         17 &    31 &   27.2 &   99.5 &   0.929 &   1.0 &  -1.1 &  15.5 &   6.9 \\ \hline
         16 &    33 &   36.7 &   81.7 &   0.484 &   2.3 &  -2.0 &  21.5 &  10.7 \\ \hline
\end{tabular}
\end{center}
\caption[Swimming details for datasets V and VI]
{Purity ($P$), efficiency ($E$), swimming factors ($F_{\rm sw}$), swimming uncertainties ($\delta^{+} F_{\rm sw}$, $\delta^{-} F_{\rm sw}$), 
uncorrelated experimental uncertainties ($\delta_{uncor}$) and the ratio of the swimming uncertainty to the experimental uncorrelated one ($\delta F_{\rm sw}/\delta_{uncor}$) 
for the \Dstar double-differential cross sections for datasets V and VI. The bin numbering scheme is consistent with Figs.~\ref{fig:comb:dstar:double:swimzd97_1} to~\ref{fig:comb:dstar:double:swimhera1h1_1}.}
\label{tab:comb:dstar:double:swimh1hera1}
\end{table}


==> content/combination/dstar/tabs/swimming/swimming_zeus9800_reduced.tex <==
\begin{table}[tbp]
\begin{center}
\tabcolsep1.1mm
\renewcommand*{\arraystretch}{1.2}
%\begin{tabular}{|l|l|l|l|l|l|l|l|l|} \hline
\begin{tabular}{|l|l|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|} \hline
%Input bin & Output bin & $P$ [\%]    & $E$ [\%] & $F_{\rm sw}$ & $\delta^{+} F_{\rm sw}$ & $\delta^{-} F_{\rm sw}$ [\%] & $\delta_{uncor}$ [\%] &  $\delta F_{\rm sw}/\delta_{uncor}$  [\%] \\ \hline
Input bin & Output bin & P~[\%]    & E~[\%] & F_{\rm sw} & \delta^{+} F_{\rm sw} & \delta^{-} F_{\rm sw}~[\%] & \delta_{uncor}~[\%] &  \delta F_{\rm sw}/\delta_{uncor}~[\%] \\ \hline
          1 &        1 &  100.0 &  100.0 &   1.000 &   0.0 &  -0.0 &  13.0 &   0.0 \\ \hline
          2 &        2 &   81.4 &  100.0 &   1.046 &   0.1 &  -0.5 &  11.3 &   4.1 \\ \hline
          3 &        3 &   95.4 &   82.8 &   1.080 &   0.7 &  -0.5 &  12.1 &   5.6 \\ \hline
          4 &        4 &  100.0 &   94.8 &   1.027 &   0.2 &  -0.2 &  20.7 &   0.9 \\ \hline
          5 &        5 &   73.6 &   86.7 &   1.094 &   1.1 &  -0.9 &  11.4 &   9.6 \\ \hline
          6 &        6 &   52.4 &  100.0 &   1.127 &   0.8 &  -0.4 &   7.9 &  10.5 \\ \hline
          7 &        7 &   70.5 &   82.7 &   1.200 &   0.6 &  -0.8 &  20.3 &   4.1 \\ \hline
          8 &        8 &   73.9 &   94.8 &   1.145 &   0.3 &  -0.6 &  14.7 &   3.8 \\ \hline
          9 &       10 &   50.8 &   50.2 &   1.091 &   6.3 &  -4.3 &  12.4 &  50.5 \\ \hline
         10 &       11 &   48.9 &   64.9 &   1.304 &   0.9 &  -0.9 &  11.3 &   8.2 \\ \hline
         11 &       13 &   68.5 &   64.7 &   0.895 &   1.8 &  -1.1 &  19.1 &   9.7 \\ \hline
         12 &       15 &   51.5 &   76.9 &   1.007 &   5.5 &  -4.0 &  10.3 &  53.4 \\ \hline
         13 &       16 &   62.0 &  100.0 &   1.062 &   0.2 &  -0.5 &   8.4 &   6.5 \\ \hline
         14 &       17 &   85.8 &   67.2 &   1.194 &   1.0 &  -1.5 &  17.1 &   8.8 \\ \hline
         15 &       18 &  100.0 &   84.7 &   1.088 &   0.3 &  -0.5 &  17.6 &   3.1 \\ \hline
         16 &       20 &   53.5 &   71.0 &   1.007 &   4.9 &  -4.0 &  11.0 &  44.9 \\ \hline
         17 &       21 &   61.8 &   92.2 &   1.019 &   0.6 &  -0.1 &  10.7 &   5.6 \\ \hline
         18 &       22 &   85.5 &   62.5 &   1.137 &   0.8 &  -1.1 &  27.1 &   4.0 \\ \hline
         19 &       23 &  100.0 &   77.4 &   1.053 &   0.8 &  -0.6 &  28.6 &   2.8 \\ \hline
         20 &       25 &   51.3 &   97.6 &   1.053 &   2.5 &  -2.3 &  11.3 &  21.7 \\ \hline
         21 &       26 &   51.5 &   81.7 &   1.080 &   0.7 &  -0.6 &   8.6 &   7.9 \\ \hline
         22 &       27 &   75.2 &   53.7 &   1.137 &   0.1 &  -1.1 &  11.6 &   9.9 \\ \hline
         23 &       28 &   92.4 &   82.3 &   1.035 &   0.6 &  -0.7 &  14.7 &   4.9 \\ \hline
         24 &       31 &   43.1 &   67.5 &   0.915 &   3.2 &  -2.8 &  11.8 &  27.1 \\ \hline
         25 &       32 &   79.0 &   72.4 &   0.799 &   0.3 &  -0.3 &  17.8 &   1.8 \\ \hline
         26 &       33 &   79.2 &   90.0 &   0.812 &   0.7 &  -0.2 &  24.7 &   2.7 \\ \hline
      27,28 &       34 &   61.1 &   88.8 &   1.130 &   0.6 &  -0.3 &  25.8 &   2.2 \\ \hline
         29 &       35 &   51.3 &   99.5 &   1.082 &   0.1 &  -0.9 &  32.4 &   2.7 \\ \hline
         30 &       38 &   59.8 &   76.7 &   0.730 &   0.8 &  -0.8 &  25.6 &   3.1 \\ \hline
         31 &       39 &   62.1 &   95.1 &   0.746 &   0.4 &  -0.5 &  26.1 &   1.8 \\ \hline
\end{tabular}
\end{center}
\caption[Swimming details for datasets IV]
{Purity ($P$), efficiency ($E$), swimming factors ($F_{\rm sw}$), swimming uncertainties ($\delta^{+} F_{\rm sw}$, $\delta^{-} F_{\rm sw}$), 
uncorrelated experimental uncertainties ($\delta_{uncor}$) and the ratio of the swimming uncertainty to the experimental uncorrelated one ($\delta F_{\rm sw}/\delta_{uncor}$) 
for the \Dstar double-differential cross sections for dataset IV. The bin numbering scheme is consistent with Figs.~\ref{fig:comb:dstar:double:swimzd00_1} to~\ref{fig:comb:dstar:double:swimzd00_1}.}
\label{tab:comb:dstar:double:swimzd00}
\end{table}


==> content/combination/dstar/tabs/swimming/swimming_zeushera2_reduced.tex <==
\begin{table}[tbp]
\begin{center}
\tabcolsep1.1mm
\renewcommand*{\arraystretch}{1.12}
%\begin{tabular}{|l|l|l|l|l|l|l|l|l|} \hline
\begin{tabular}{|l|l|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|>{$}r<{$}|} \hline
%Input bin & Output bin & $P$ [\%]    & $E$ [\%] & $F_{\rm sw}$ & $\delta^{+} F_{\rm sw}$ & $\delta^{-} F_{\rm sw}$ [\%] & $\delta_{uncor}$ [\%] &  $\delta F_{\rm sw}/\delta_{uncor}$  [\%] \\ \hline
Input bin & Output bin & P~[\%]    & E~[\%] & F_{\rm sw} & \delta^{+} F_{\rm sw} & \delta^{-} F_{\rm sw}~[\%] & \delta_{uncor}~[\%] &  \delta F_{\rm sw}/\delta_{uncor}~[\%] \\ \hline
          1 &        9 &   83.1 &  100.0 &   0.948 &   0.3 &  -0.0 &  28.4 &   1.1 \\ \hline
          2 &       10 &   83.2 &  100.0 &   0.949 &   0.2 &  -0.3 &  13.3 &   2.3 \\ \hline
          3 &       11 &   83.2 &  100.0 &   0.949 &   0.2 &  -0.4 &   7.3 &   5.9 \\ \hline
          4 &       12 &   83.2 &  100.0 &   0.950 &   0.1 &  -0.3 &   6.7 &   4.4 \\ \hline
          5 &       13 &   83.1 &  100.0 &   0.948 &   0.2 &  -0.3 &   7.5 &   3.8 \\ \hline
          6 &       14 &  100.0 &  100.0 &   1.000 &   0.0 &  -0.0 &  16.1 &   0.0 \\ \hline
          7 &       15 &  100.0 &  100.0 &   1.000 &   0.0 &  -0.0 &   7.8 &   0.0 \\ \hline
          8 &       16 &  100.0 &  100.0 &   1.000 &   0.0 &  -0.0 &   6.4 &   0.0 \\ \hline
          9 &       17 &  100.0 &  100.0 &   1.000 &   0.0 &  -0.0 &   5.5 &   0.0 \\ \hline
         10 &       18 &  100.0 &  100.0 &   1.000 &   0.0 &  -0.0 &   7.5 &   0.0 \\ \hline
         11 &       19 &  100.0 &  100.0 &   1.000 &   0.0 &  -0.0 &  16.9 &   0.0 \\ \hline
         12 &       20 &  100.0 &  100.0 &   1.000 &   0.0 &  -0.0 &   7.3 &   0.0 \\ \hline
         13 &       21 &  100.0 &  100.0 &   1.000 &   0.0 &  -0.0 &   6.2 &   0.0 \\ \hline
         14 &       22 &  100.0 &  100.0 &   1.000 &   0.0 &  -0.0 &   6.4 &   0.0 \\ \hline
         15 &       23 &  100.0 &  100.0 &   1.000 &   0.0 &  -0.0 &   8.4 &   0.0 \\ \hline
         16 &       24 &  100.0 &  100.0 &   1.000 &   0.0 &  -0.0 &  32.6 &   0.0 \\ \hline
         17 &       25 &  100.0 &  100.0 &   1.000 &   0.0 &  -0.0 &   7.4 &   0.0 \\ \hline
         18 &       26 &  100.0 &  100.0 &   1.000 &   0.0 &  -0.0 &   5.5 &   0.0 \\ \hline
         19 &       27 &  100.0 &  100.0 &   1.000 &   0.0 &  -0.0 &   5.3 &   0.0 \\ \hline
         20 &       28 &  100.0 &  100.0 &   1.000 &   0.0 &  -0.0 &   6.7 &   0.0 \\ \hline
         21 &       29 &  100.0 &  100.0 &   1.000 &   0.0 &  -0.0 &  40.5 &   0.0 \\ \hline
         22 &       30 &  100.0 &  100.0 &   1.000 &   0.0 &  -0.0 &  12.6 &   0.0 \\ \hline
         23 &       31 &  100.0 &  100.0 &   1.000 &   0.0 &  -0.0 &   8.7 &   0.0 \\ \hline
         24 &       32 &  100.0 &  100.0 &   1.000 &   0.0 &  -0.0 &   6.6 &   0.0 \\ \hline
         25 &       33 &  100.0 &  100.0 &   1.000 &   0.0 &  -0.0 &   8.5 &   0.0 \\ \hline
         26 &       34 &   93.0 &  100.0 &   1.023 &   0.2 &  -0.2 &  12.2 &   1.9 \\ \hline
         27 &       35 &  100.0 &   87.4 &   1.052 &   0.2 &  -0.0 &  17.0 &   1.3 \\ \hline
         28 &       36 &  100.0 &  100.0 &   1.000 &   0.0 &  -0.0 &  14.5 &   0.0 \\ \hline
         29 &       37 &  100.0 &  100.0 &   1.000 &   0.0 &  -0.0 &  17.5 &   0.0 \\ \hline
         30 &       38 &   92.6 &  100.0 &   0.983 &   0.5 &  -0.0 &  25.1 &   1.9 \\ \hline
         31 &       39 &  100.0 &   95.2 &   1.015 &   0.0 &  -0.2 &  21.8 &   1.1 \\ \hline
\end{tabular}
\end{center}
\caption[Swimming details for datasets I--III]
{Purity ($P$), efficiency ($E$), swimming factors ($F_{\rm sw}$), swimming uncertainties ($\delta^{+} F_{\rm sw}$, $\delta^{-} F_{\rm sw}$), 
uncorrelated experimental uncertainties ($\delta_{uncor}$) and the ratio of the swimming uncertainty to the experimental uncorrelated one ($\delta F_{\rm sw}/\delta_{uncor}$) 
for the \Dstar double-differential cross sections for datasets I--III. The bin numbering scheme is consistent with Figs.~\ref{fig:comb:dstar:double:swimhera2_1} to~\ref{fig:comb:dstar:double:swimhera1h1_4}.}
\label{tab:comb:dstar:double:swimhera2}
\end{table}


==> content/combination/dstar/tabs/tab_eta.tex <==
\begin{table}[t]
\begin{center}
\tabcolsep2.1mm
\renewcommand*{\arraystretch}{1.2}
\begin{tabular}{|c|c|c|c|c|}
\hline
$\eta(\Dstar)$ &$ \frac{d\sigma}{d\eta(\Dstar)}$ &$\delta_{unc}$  &$\delta_{cor}$&$\delta_{tot}$ \\
         & (nb)                         &$(\%)$            &$(\%)$ &$(\%)$ \\ 
\hline
-1.50 : -1.25 & 1.36 & 5.8 & 4.3 & 7.2 \\ \hline
-1.25 : -1.00 & 1.52 & 4.6 & 4.0 & 6.1 \\ \hline
-1.00 : -0.75 & 1.59 & 4.6 & 4.0 & 6.1 \\ \hline
-0.75 : -0.50 & 1.79 & 3.8 & 3.5 & 5.2 \\ \hline
-0.50 : -0.25 & 1.83 & 3.8 & 3.3 & 5.1 \\ \hline
-0.25 : 0.00 & 1.89 & 3.8 & 3.7 & 5.3 \\ \hline
0.00 : 0.25 & 1.86 & 4.0 & 3.4 & 5.2 \\ \hline
0.25 : 0.50 & 1.88 & 4.0 & 3.6 & 5.4 \\ \hline
0.50 : 0.75 & 1.91 & 4.1 & 3.5 & 5.4 \\ \hline
0.75 : 1.00 & 1.92 & 4.3 & 4.0 & 5.9 \\ \hline
1.00 : 1.25 & 2.08 & 4.7 & 4.0 & 6.1 \\ \hline
1.25 : 1.50 & 1.81 & 6.3 & 4.8 & 7.9 \\ \hline
\end{tabular}
\end{center}
\caption{The combined differential \Dstar cross section as a function of $\eta(\Dstar)$, with its 
uncorrelated ($\delta_{unc}$), correlated ($\delta_{cor}$) and total ($\delta_{tot}$) uncertainties.}
\label{tab:result_eta}
\end{table}


==> content/combination/dstar/tabs/tab_input.tex <==
\begin{table}[t]
\caption{Datasets used in the combination of the visible \Dstar cross sections. For each dataset the respective kinematic region 
and the integrated luminosity, ${\cal L}$, are given.}
\label{tab:comb:dstar:input}
\begin{center}
\tabcolsep1.1mm
\renewcommand*{\arraystretch}{1.2}
\begin{tabular}{|l|l|l|l|l|l|}
\hline
\multirow{3}{*}{Dataset} & \multicolumn{4}{|c|}{Kinematic range}      & ${\cal L}$  \\ \cline{2-5}
                          & $Q^2$        & $y$ & $p_T(\Dstar)$ & $\eta(\Dstar)$ & \\ 
                          & [$\SI{}{GeV}^{2}$] &     & [$\SI{}{GeV}$]     &             & [$\text{pb}^{\text{-1}}$]            \\ \hline
I:\ \ \  H1 $\Dstar$ HERA-II (medium $Q^2$) \cite{h1dstar_hera2} & $~~~~5:100$ & $0.02:0.70$ & $1.5:\infty$ & $-1.5:1.5$ & $348$ \\ \hline
II:\ \  H1 $\Dstar$ HERA-II (high $Q^2$) \cite{h1dstarhighQ2} & $100:1000$ & $0.02:0.70$ & $1.5:\infty$ & $-1.5:1.5$ & $351$ \\ \hline
III: ZEUS $\Dstar$ HERA-II \cite{zeusdstar_hera2} & $~~~~5:1000$ & $0.02:0.70$ & $1.5:20.0$ & $-1.5:1.5$ & $363$ \\ \hline
IV:\ ZEUS $\Dstar$ HERA-I \cite{zd00} & $~1.5:1000$ & $0.02:0.70$ & $1.5:15.0$ & $-1.5:1.5$ & $82$ \\ \hline
\end{tabular}
\end{center}
\end{table}


==> content/combination/dstar/tabs/tab_pt.tex <==
\begin{table}[t]
\begin{center}
\tabcolsep2.1mm
\renewcommand*{\arraystretch}{1.2}
\begin{tabular}{|c|c|c|c|c|}
\hline
$p_T(\Dstar)$ &$ \frac{d\sigma}{dp_T(\Dstar)}$ &$\delta_{unc}$  &$\delta_{cor}$&$\delta_{tot}$ \\
  ($\SI{}{GeV}$)       & ($\SI{}{nb/GeV}$)                         &$(\%)$            &$(\%)$ &$(\%)$ \\ 
\hline
1.50 : 1.88 & 2.35 & 6.4 & 4.7 & 8.0 \\ \hline
1.88 : 2.28 & 2.22 & 4.9 & 4.2 & 6.4 \\ \hline
2.28 : 2.68 & 1.98 & 3.7 & 4.0 & 5.5 \\ \hline
2.68 : 3.08 & 1.55 & 3.5 & 3.7 & 5.1 \\ \hline
3.08 : 3.50 & 1.20 & 3.7 & 3.5 & 5.1 \\ \hline
3.50 : 4.00 & 9.29 $\times 10^{-1}$ & 3.2 & 3.4 & 4.7 \\ \hline
4.00 : 4.75 & 6.14 $\times 10^{-1}$ & 3.0 & 3.5 & 4.6 \\ \hline
4.75 : 6.00 & 3.19 $\times 10^{-1}$ & 3.1 & 3.3 & 4.5 \\ \hline
6.00 : 8.00 & 1.15 $\times 10^{-1}$ & 3.8 & 3.7 & 5.3 \\ \hline
8.00 : 11.00 & 3.32 $\times 10^{-2}$ & 5.4 & 3.7 & 6.5 \\ \hline
11.00 : 20.00 & 3.80 $\times 10^{-3}$ & 10.4 & 6.4 & 12.2 \\ \hline
\end{tabular}
\end{center}
\caption{The combined differential \Dstar cross section as a function of $p_T(\Dstar)$, with its 
uncorrelated ($\delta_{unc}$), correlated ($\delta_{cor}$) and total ($\delta_{tot}$) uncertainties.} 
\label{tab:result_pt}
\end{table}


==> content/combination/dstar/tabs/tab_q2.tex <==
\begin{table}[t]
\begin{center}
\tabcolsep2.1mm
\renewcommand*{\arraystretch}{1.2}
\begin{tabular}{|c|c|c|c|c|}
\hline
$Q^2$ &$ \frac{d\sigma}{dQ^2}$ &$\delta_{unc}$  &$\delta_{cor}$&$\delta_{tot}$ \\
  ($\SI{}{GeV}^2$)       & ($\SI{}{GeV}^2$)                         &$(\%)$            &$(\%)$ &$(\%)$ \\ 
\hline
5 : 8 & 4.74 $\times 10^{-1}$ & 4.0 & 5.0 & 6.4 \\ \hline
8 : 10 & 2.96 $\times 10^{-1}$ & 4.3 & 3.8 & 5.8 \\ \hline
10 : 13 & 2.12 $\times 10^{-1}$ & 3.8 & 4.0 & 5.6 \\ \hline
13 : 19 & 1.24 $\times 10^{-1}$ & 3.2 & 3.8 & 5.0 \\ \hline
19 : 28 & 7.26 $\times 10^{-2}$ & 3.5 & 3.6 & 5.0 \\ \hline
28 : 40 & 3.97 $\times 10^{-2}$ & 3.7 & 4.0 & 5.5 \\ \hline
40 : 60 & 1.64 $\times 10^{-2}$ & 4.4 & 4.7 & 6.4 \\ \hline
60 : 100 & 7.45 $\times 10^{-3}$ & 5.2 & 3.9 & 6.5 \\ \hline
100 : 158 & 2.08 $\times 10^{-3}$ & 7.2 & 5.3 & 9.0 \\ \hline
158 : 251 & 8.82 $\times 10^{-4}$ & 7.6 & 5.0 & 9.1 \\ \hline
251 : 1000 & 7.50 $\times 10^{-5}$ & 12.0 & 6.7 & 13.3 \\ \hline
\end{tabular}
\end{center}
\caption{The combined differential \Dstar cross section as a function of $Q^2$, with its 
%The values of the cross section are presented together 
%with 
uncorrelated ($\delta_{unc}$), correlated ($\delta_{cor}$) and total ($\delta_{tot}$) uncertainties.}
%The total uncertainty ($\delta_{tot}$) is obtained by adding the uncorrelated and correlated uncertainties in quadrature.}
\label{tab:result_q2}
\end{table}


==> content/combination/dstar/tabs/tab_q2y.tex <==
\begin{table}[t]
\begin{center}
\tabcolsep2.1mm
\renewcommand*{\arraystretch}{1.1}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
$Q^2$ & $y$ & $ \frac{d^2\sigma}{dQ^2dy}$ &$\delta_{unc}$  &$\delta_{cor}$&$\delta_{tot}$ \\
  (\gev$^{2}$)  &     & (nb/\gev$^{2}$)                         &$(\%)$            &$(\%)$ &$(\%)$ \\ 
\hline
1.5 : 3.5 & 0.02 : 0.09 & 4.76 & 12.9 & 2.5 & 13.2 \\
        & 0.09 : 0.16 & 5.50 & 11.3 & 2.6 & 11.5 \\
        & 0.16 : 0.32 & 3.00 & 12.0 & 2.6 & 12.3 \\
        & 0.32 : 0.70 & 9.21 $\times 10^{-1}$ & 20.5 & 2.5 & 20.7 \\ \hline
3.5 : 5.5 & 0.02 : 0.09 & 2.22 & 11.3 & 2.8 & 11.6 \\
        & 0.09 : 0.16 & 1.98 & 7.9 & 2.7 & 8.3 \\
        & 0.16 : 0.32 & 1.09 & 20.2 & 2.7 & 20.4 \\
        & 0.32 : 0.70 & 3.47 $\times 10^{-1}$ & 14.6 & 2.6 & 14.8 \\ \hline
5.5 : 9 & 0.02 : 0.05 & 1.06 & 12.3 & 4.4 & 13.1 \\
        & 0.05 : 0.09 & 1.46 & 7.8 & 4.1 & 8.8 \\
        & 0.09 : 0.16 & 1.32 & 5.4 & 4.3 & 6.9 \\
        & 0.16 : 0.32 & 7.73 $\times 10^{-1}$ & 4.9 & 3.9 & 6.3 \\
        & 0.32 : 0.70 & 2.51 $\times 10^{-1}$ & 5.6 & 4.2 & 7.0 \\ \hline
9 : 14 & 0.02 : 0.05 & 5.20 $\times 10^{-1}$ & 13.0 & 6.6 & 14.6 \\
        & 0.05 : 0.09 & 7.68 $\times 10^{-1}$ & 6.6 & 3.9 & 7.7 \\
        & 0.09 : 0.16 & 5.69 $\times 10^{-1}$ & 4.6 & 2.8 & 5.4 \\
        & 0.16 : 0.32 & 4.12 $\times 10^{-1}$ & 4.6 & 3.1 & 5.6 \\
        & 0.32 : 0.70 & 1.51 $\times 10^{-1}$ & 5.6 & 4.0 & 6.9 \\ \hline
14 : 23 & 0.02 : 0.05 & 2.29 $\times 10^{-1}$ & 11.4 & 6.3 & 13.0 \\
        & 0.05 : 0.09 & 3.78 $\times 10^{-1}$ & 6.5 & 4.1 & 7.7 \\
        & 0.09 : 0.16 & 2.90 $\times 10^{-1}$ & 4.8 & 3.3 & 5.8 \\
        & 0.16 : 0.32 & 1.86 $\times 10^{-1}$ & 5.0 & 3.4 & 6.0 \\
        & 0.32 : 0.70 & 6.92 $\times 10^{-2}$ & 6.2 & 4.4 & 7.7 \\ \hline
23 : 45 & 0.02 : 0.05 & 6.91 $\times 10^{-2}$ & 14.8 & 8.2 & 16.7 \\
        & 0.05 : 0.09 & 1.23 $\times 10^{-1}$ & 5.9 & 3.6 & 6.9 \\
        & 0.09 : 0.16 & 1.14 $\times 10^{-1}$ & 4.4 & 3.0 & 5.3 \\
        & 0.16 : 0.32 & 7.42 $\times 10^{-2}$ & 4.3 & 3.0 & 5.2 \\
        & 0.32 : 0.70 & 3.21 $\times 10^{-2}$ & 5.2 & 3.7 & 6.4 \\ \hline
45 : 100 & 0.02 : 0.05 & 6.16 $\times 10^{-3}$ & 33.5 & 11.1 & 35.3 \\
        & 0.05 : 0.09 & 2.70 $\times 10^{-2}$ & 11.0 & 4.4 & 11.8 \\
        & 0.09 : 0.16 & 2.05 $\times 10^{-2}$ & 8.0 & 3.7 & 8.8 \\
        & 0.16 : 0.32 & 1.99 $\times 10^{-2}$ & 5.4 & 3.2 & 6.3 \\
        & 0.32 : 0.70 & 7.84 $\times 10^{-3}$ & 6.9 & 4.0 & 7.9 \\ \hline
100 : 158 & 0.02 : 0.32 & 4.12 $\times 10^{-3}$ & 8.2 & 4.1 & 9.2 \\
        & 0.32 : 0.70 & 2.18 $\times 10^{-3}$ & 11.1 & 4.1 & 11.9 \\ \hline
158 : 251 & 0.02 : 0.30 & 1.79 $\times 10^{-3}$ & 10.2 & 4.4 & 11.1 \\
        & 0.30 : 0.70 & 9.28 $\times 10^{-4}$ & 11.6 & 4.6 & 12.5 \\ \hline
251 : 1000 & 0.02 : 0.26 & 1.31 $\times 10^{-4}$ & 14.5 & 4.7 & 15.3 \\
        & 0.26 : 0.70 & 1.18 $\times 10^{-4}$ & 12.7 & 5.0 & 13.6 \\ \hline
\end{tabular}
\end{center}
\caption{The combined double-differential \Dstar cross section as a function of $Q^2$ and $y$, with its 
uncorrelated ($\delta_{unc}$), correlated ($\delta_{cor}$) and total ($\delta_{tot}$) uncertainties.}
\label{tab:result_q2y}
\end{table}


==> content/combination/dstar/tabs/tab_y.tex <==
\begin{table}[t]
\begin{center}
\tabcolsep2.1mm
\renewcommand*{\arraystretch}{1.2}
\begin{tabular}{|c|c|c|c|c|}
\hline
$y$ &$ \frac{d\sigma}{dy}$ &$\delta_{unc}$  &$\delta_{cor}$&$\delta_{tot}$ \\
         & (nb)                         &$(\%)$            &$(\%)$ &$(\%)$ \\ 
\hline
0.02 : 0.05 & 12.13 & 5.8 & 9.1 & 10.8 \\ \hline
0.05 : 0.09 & 18.84 & 3.9 & 4.6 & 6.0 \\ \hline
0.09 : 0.13 & 16.99 & 3.4 & 4.3 & 5.5 \\ \hline
0.13 : 0.18 & 13.35 & 3.7 & 4.2 & 5.6 \\ \hline
0.18 : 0.26 & 11.19 & 3.4 & 3.7 & 5.0 \\ \hline
0.26 : 0.36 & 7.65 & 3.7 & 4.2 & 5.6 \\ \hline
0.36 : 0.50 & 4.78 & 4.0 & 5.3 & 6.6 \\ \hline
0.50 : 0.70 & 2.65 & 5.6 & 6.4 & 8.5 \\ \hline
\end{tabular}
\end{center}
\caption{The combined differential \Dstar cross section as a function of $y$, with its 
uncorrelated ($\delta_{unc}$), correlated ($\delta_{cor}$) and total ($\delta_{tot}$) uncertainties.}
\label{tab:result_y}
\end{table}


==> content/combination/dstar/tabs/tab_z.tex <==
\begin{table}[t]
\begin{center}
\tabcolsep2.1mm
\renewcommand*{\arraystretch}{1.2}
\begin{tabular}{|c|c|c|c|c|}
\hline
$z(\Dstar)$ &$ \frac{d\sigma}{dz(\Dstar)}$ &$\delta_{unc}$  &$\delta_{cor}$&$\delta_{tot}$ \\
         & (nb)                         &$(\%)$            &$(\%)$ &$(\%)$ \\ 
\hline
0.00 : 0.10 & 3.28 & 9.5 & 5.9 & 11.2 \\ \hline
0.10 : 0.20 & 7.35 & 4.8 & 6.3 & 7.9 \\ \hline
0.20 : 0.32 & 8.61 & 3.5 & 4.6 & 5.7 \\ \hline
0.32 : 0.45 & 8.92 & 2.7 & 3.9 & 4.7 \\ \hline
0.45 : 0.57 & 8.83 & 1.8 & 4.0 & 4.3 \\ \hline
0.57 : 0.80 & 4.78 & 2.4 & 5.1 & 5.6 \\ \hline
0.80 : 1.00 & 6.31 $\times 10^{-1}$ & 8.1 & 10.2 & 13.0 \\ \hline
\end{tabular}
\end{center}
\caption{The combined differential \Dstar cross section as a function of $z(\Dstar)$, with its 
uncorrelated ($\delta_{unc}$), correlated ($\delta_{cor}$) and total ($\delta_{tot}$) uncertainties.}
\label{tab:result_z}
\end{table}

